Privacy-preserving Searchable Databases with Controllable Leakage

Searchable Encryption (SE) is a technique that allows Cloud Service Providers (CSPs) to search over encrypted datasets without learning the content of queries and records. In recent years, many SE schemes have been proposed to protect outsourced data from CSPs. Unfortunately, most of them leak sensitive information, from which the CSPs could still infer the content of queries and records by mounting leakage-based inference attacks, such as the count attack and file injection attack. In this work, first we define the leakage in searchable encrypted databases and analyse how the leakage is leveraged in existing leakage-based attacks. Second, we propose a Privacy-preserving Multi-cloud based dynamic symmetric SE (SSE) scheme for relational Database (P-McDb). P-McDb has minimal leakage, which not only ensures confidentiality of queries and records, but also protects the search, access, and size patterns from CSPs. Moreover, P-McDb ensures both forward and backward privacy of the database. Thus, P-McDb could resist existing leakage-based attacks, e.g., active file/record-injection attacks. We give security definition and analysis to show how P-McDb hides the aforementioned patterns. Finally, we implemented a prototype of P-McDb and test it using the TPC-H benchmark dataset. Our evaluation results show the feasibility and practical efficiency of P-McDb.

==> PMcDb_arXiv/abstract.tex <==
\begin{abstract}
%In cloud computing,
Searchable Encryption (SE) is a technique that allows Cloud Service Providers (CSPs) to search over encrypted datasets without learning the content of queries and records.
In recent years, many SE schemes have been proposed to protect outsourced data from CSPs.
Unfortunately, most of them leak sensitive information, from which the CSPs could still infer the content of queries and records by mounting leakage-based inference attacks, such as the \emph{count attack} and \emph{file injection attack}.

In this work, first we define the leakage in searchable encrypted databases and analyse how the leakage is leveraged in existing leakage-based attacks.
Second, we propose a \underline{P}rivacy-preserving \underline{M}ulti-\underline{c}loud based dynamic symmetric SE (SSE) scheme for relational \underline{D}ata\underline{b}ase (\framework).
\framework has minimal leakage, which not only ensures confidentiality of queries and records, but also protects the search, access, and size patterns from CSPs.
Moreover, \framework ensures both forward and backward privacy of the database.
Thus, \framework could resist existing leakage-based attacks, \eg active file/record-injection attacks.
%\framework also supports multi-user access without re-generating a new key and re-encrypting the data for user revocation.
We give security definition and analysis to show how \framework hides the aforementioned patterns.
Finally, we implemented a prototype of \framework and test it using the TPC-H benchmark dataset.
Our evaluation results show the feasibility and practical efficiency of \framework.
%}
\end{abstract}


==> PMcDb_arXiv/sections/attacks.tex <==
\begin{table}
\scriptsize
  \centering
   \caption{Summary of leakage profiles and attacks against encrypted databases}
   \label{tbl:summary}
  \begin{tabular}{|c|l|l|}
     \hline
     % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
    \textbf{Leakage}  & \textbf{Schemes} & \textbf{Attacks} \\ \hline
    $\mathcal{L}_3$
    &
\begin{tabular}[c]{@{}l@{}}
    CryptDB \cite{Popa:2011:Cryptdb} \\
    DBMask \cite{Sarfraz:2015:DBMask} \\
    Cipherbase \cite{Arasu:CIDR13:Cipherbase}\\
    Monomi \cite{Tu:PVLDB13:monomi} \\
    Seabed \cite{Papadimitriou:usenix2016:Seabed} \\
\end{tabular}

& \begin{tabular}[c]{@{}l@{}}
    Frequency analysis attack \\
    IKK attack \\
    Count attack \\
    Record-injection attack \\
    %Attribute recovery attack \\
    %Communication volume attack
\end{tabular} \\ \hline

$\mathcal{L}_2$
&
\begin{tabular}[c]{@{}l@{}}
     Asghar \etal \cite{Asghar:2013:CCSW} \\
     Blind Seer \cite{Fisch:SP15:BlindSeer,Pappas:BlindSeer:SP14} \\
     Arx \cite{Poddar:arx:eprint16} \\
     PPQED \cite{Samanthula:2014:Privacy}
\end{tabular}

& \begin{tabular}[c]{@{}l@{}}
    IKK attack \\
    Count attack \\
    Record-injection attack \\
    %Attribute recovery attack \\
    %Communication volume attack
\end{tabular} \\ \hline

% \multirow{2}{*}{$\mathcal{L}_1$}
$\mathcal{L}_1$
&
\begin{tabular}[c]{@{}l@{}}
    $PPQED_a$ \cite{Samanthula:2014:Privacy} \\
    SisoSPIR \cite{Ishai:2016:Private}
\end{tabular}

&
    Count attack
 \\ \hline %\\ \cline{2-3}

%$\mathcal{L}'_0$ & \framework &N/A  \\ \hline
%$\mathcal{L}_0$   & N/A        &N/A  \\ \hline

\end{tabular}
%The attacks are surveyed in Section \ref{sec:attack}.
\end{table}
%
\subsection{Attacks against SE Solutions}
\label{sec:attack}
%With the leakage profiles defined in Section \ref{sec:leakage}, the SE schemes are still provable secure under either the real-ideal \cite{Curtmola:2006:Searchable,Chang:2005:PPK}, Universal Composable (UC) \cite{Kurosawa:FC2012:UC} or other specific security models.
%However, in practice, the leakage can be exploited to recover the content of records and queries.
In recent years, leakage-based attacks against SE schemes have been investigated in the literature.
Table \ref{tbl:summary} summarises the existing SE solutions for relational databases and the attacks applicable to them.
In the following, we illustrate how the existing leakage-based attacks could recover the data and queries.
Specifically, for each attack, we analyse its leveraged leakage, required knowledge, process, and consequences.
% in file storage and relational database SE solutions. Moreover, we customise the attacks mounted on file collections to the encrypted databases.

\subsubsection{Frequency Analysis Attack}
In \cite{Naveed:2015:Inference}, Naveed \etal describe an attack on PPE-based SE schemes, where the CSP could recover encrypted records by analysing the leaked frequency information, \ie data distribution.
To succeed in this attack, in addition to the encrypted database, the CSP also requires some auxiliary information, such as the application background, publicly available statistics, and prior versions of the targeted database.
%In practice, such auxiliary information could be obtained by accessing the application, from documentations or through a prior data breach.
%Moreover, publicly available statistics, \eg census data or hospital statistics, can be obtained online.
In PPE-based SE schemes, the frequency information of an encrypted database is equal to that of the database in plaintext.
By comparing the leaked frequency information with the obtained statistics relevant to the application, the CSP could recover the encrypted data elements stored in encrypted databases.
%For instance, most of the organisations, such as universities, publish their staff lists in their homepages, from which the CSP can learn the statistics of names in the targeted organisations.
%Moreover, the CSP knows the owner of each encrypted database by nature.
%By comparing the leaked frequency information with the owner organisation's statistics of names, the CSP can infer the name of each record in the encrypted database.
%Specifically, the field whose element distribution is close to the known name distribution could be `Name'.
%Furthermore, the element with the highest occurrence could be the most popular name in the organisation, and so forth.
In \cite{Naveed:2015:Inference}, Naveed \etal recovered more than $60\%$ of records when evaluating this attack with real electronic medical records using CryptDB.
We stress that this attack does not require any queries or interaction with users.
The encrypted databases with $\mathcal{L}_3$ leakage profile, \ie PPE-based databases, such as CryptDB and DBMask, are vulnerable to this attack.
%The specific leakage the attacker need to know is the frequency of encrypted data.

\subsubsection{IKK Attack}
IKK attack proposed by Islam \etal \cite{Islam:2012:Access} is the first attack exploiting the access pattern leakage.
The goal of the IKK attack is to recover encrypted queries in encrypted file collection systems, \ie recover the plaintext of searched keywords.
Note that this attack can also be used to recover queries in encrypted databases since it does not leverage the leakage specific to file collections.
In this attack, the CSP needs to know possible keywords in the dataset and the expected probability of any two keywords appearing in a file (\ie co-occurrence probability).
%, and even a set of queries in plaintext (yet not a must).
%Again, obtaining such information is not a hard task if the CSP knows the application scenario.
%For instance, if the targeted files are from a university, `lecture', `workshop' and `tutorial' could be the possible keywords.
%The CSP can also simulate the expected co-occurrence probability of any two keywords by carrying out a probabilistic analysis over publicly available online datasets, such as the news and documents published in the university's website.
Formally, the CSP guesses $m$ potential keywords and builds an $m\times m$ matrix $\tilde{C}$ whose element is the co-occurrence probability of each keyword pair.
The CSP mounts the IKK attack by observing the access pattern revealed by the encrypted queries.
Specifically, by checking if any two queries match the same files or not, the number of files containing any two searched keywords (\ie the co-occurrence rate) can be reconstructed.
Assume the CSP observes $n$ queries.
It constructs an $n \times n$ matrix $C$ with their co-occurrence rates.
By using the simulated annealing technique \cite{KirkpatrickGV83}, the CSP can find the best match between $\tilde{C}$ and $C$ and map the encrypted keywords to the guesses.
In \cite{Islam:2012:Access}, Islam \etal mounted the IKK attack over the Enron email dataset \cite{eronemail:2017} and recovered $80\%$ of the queries with certain vocabulary sizes.
The encrypted relational databases with leakage profile $\mathcal{L}_2$ or $\mathcal{L}_1$, such as Arx \cite{Poddar:arx:eprint16}, Blind Seer \cite{Pappas:BlindSeer:SP14}, and PPQED \cite{Samanthula:2014:Privacy}, are also vulnerable to the IKK attack.
%To mount the IKK attack on databases, the CSP needs to guess the co-occurrences of any two elements in two different fields in the real database based on some background knowledge of the application.
%The encrypted queries can be recovered by observing the revealed access pattern and comparing them with the known dataset.

%\textred{Note that the PPE-based SE solutions are also vulnerable to the IKK attack since they leak all the $\mathcal{L}_2$ profiles after searching.}

\subsubsection{File-injection and Record-injection Attack}
The file-injection attack \cite{Zhang:2016:All} is an active attack mounted on encrypted file collections, which is also named as \emph{chosen-document attack} in \cite{Cash:2015:leakage}.
%All the other leakage-based attacks mentioned in this work are passive attacks, where CSPs only get some auxiliary information and observe the search operation performed on the CSP.
%In file-injection attack, the CSP could actively trick users into inserting files of its choice.
The file-injection attack attempts to recover encrypted queries by exploiting access pattern in encrypted file storage.
More recently, Abdelraheem \etal \cite{Abdelraheem:eprint17:record} extended this attack to encrypted databases and defined it as \emph{record-injection attack}.
Compared with the IKK and count attack (will be discussed in Section \ref{subsec:conut}), much less auxiliary knowledge is required: the CSP only needs to know the keywords universe of the system.
In \cite{Zhang:2016:All}, Zhang \etal presented the first concrete file-injection attack and showed that the encrypted queries can be revealed with a small set of injected files.
Specifically, in this attack, the CSP (acting as an active attacker) sends files composed of the keywords of its choice, such as emails, to users who then encrypt and upload them to the CSP, which are called \emph{injected files}.
If no other files are uploaded simultaneously, the CSP can easily know the storage location of each injected file.
Moreover, the CSP can check which injected files match the subsequent queries.
Given enough injected files with different keyword combinations, the CSP could recover the keyword included in a query by checking the search result.
%Specifically, the keywords included in the matched but not included in the unmatched injected files are the possible searched keywords.
The encrypted databases with $\mathcal{L}_2$ or $\mathcal{L}_3$ leakage profiles are vulnerable to this attack.
Although some works \cite{BostMO17,ZuoSLSP18,ChamaniPPJ18,AmjadKM19} ensure both forward and backward privacy, they are still vulnerable to the file-injection attack due to the leakage of access pattern.
That is, after searching, the attacker could still learn the intersections between previous insert queries and the search result of current queries.
%For instance, if the injected files matching a query $Q$ all contain $w_1$ and $w_2$, but $w_2$ is also contained in other injected files that do not match $Q$, the keyword involved in $Q$ must be $w_1$.


\subsubsection{Count and Relational-count Attack}
\label{subsec:conut}
The count attack is proposed by Cash \etal in \cite{Cash:2015:leakage} to recover encrypted queries in file storage systems based on the access and size patterns leakage.
In \cite{Abdelraheem:2017:Seachable}, Abdelraheem \etal have applied this attack to databases and named it a \emph{relational-count attack}.
As in the IKK attack scenario, the CSP is also assumed to know an $m \times m$ matrix $\tilde{C}$, where its entry $\tilde{C}[w_i, w_j]$ holds the co-occurrence rate of keyword $w_i$ and $w_j$ in the targeted dataset.
In order to improve the attack efficiency and accuracy, the CSP is assumed to know, for each keyword $w$, the number of matching files $count(w)$ in the targeted dataset.
The CSP mounts the count attack by counting the number of files matching each encrypted query.
For an encrypted query, if the number of its matching files is unique and equals to a known $count(w)$, the searched keyword must be $w$.
However, if the result size of a query $EQ$ is not unique, all the keywords with $count(w)=|EDB(EQ)|$ could be the candidates.
Recall that the CSP can construct another matrix $C$ that represents the observed co-occurrence rate between any two queries based on the leakage of access pattern.
By comparing $C$ with $\tilde{C}$, the candidates for the queries with non-unique result sizes can be reduced.
With enough recovered queries, it is possible to determine the keyword of $EQ$.
In \cite{Cash:2015:leakage}, Cash \etal tested the count attack against Enron email dataset and successfully recovered almost all the queries.
The SE solutions for databases with leakage profiles above $\mathcal{L}_1$ are vulnerable to this attack.

\subsubsection{Reconstruction Attack}
In ORAM-based systems, such as SisoSPIR proposed by Ishai \etal \cite{Ishai:2016:Private}, the size and access patterns are concealed.
Unfortunately, Kellaris \etal \cite{Kellaris:ccs16:Generic} observe that the ORAM-based systems have fixed communication overhead between the CSP and users, where the length of the message sent from the CSP to the user as the result of a query is proportional to the number of records matching the query.
That is, for a query $Q$, the size of the communication sent from the CSP to the user is $\alpha |DB(Q)|+ \beta$, where $\alpha$ and $\beta$ are two constants.
In theory, by giving two (query, result) pairs, the CSP can derive $\alpha$ and $\beta$, and then infer the result sizes of other queries.
In \cite{Kellaris:ccs16:Generic}, Kellaris \etal present the \emph{reconstruction attack} that exploits the leakage of communication volume, and could reconstruct the attribute names in encrypted databases supporting range queries.
In this attack, the CSP only needs to know the underlying query distribution prior to the attack.
Their experiment illustrated that after a certain number of queries, all the attributes can be recovered in a few seconds.
Since we focus on equality queries in this work, we do not give the attack details here.
Nonetheless, after recovering the size pattern for each query, the CSP could also mount the count attack on equality queries.
%Specifically, given the occurrence of each possible keyword, the CSP could recover the queries whose result sizes are unique.
The SE schemes with $\mathcal{L}_1$ leakage profile are vulnerable to this attack.

%To the best of our knowledge, so far, no attack can recover encrypted records and queries just based on $\mathcal{L}_0$.


==> PMcDb_arXiv/sections/conclusion.tex <==
\section{Conclusions and Future Directions}
\label{sec:conclusion}
In this work, we presented the leakage profile definitions for searchable encrypted relational databases, and investigated the leakage-based attacks proposed int the literature.
We also proposed \framework, a dynamic searchable encryption scheme for multi-cloud outsourced databases.
\framework does not leak information about search, access, and size patterns.
It also achieves both forward and backward privacy, where the CSPs cannot reuse cached queries for checking if new records have been inserted or if records have been deleted.
\framework has minimal leakage, making it resistant to exiting leakage-based attacks. %, including the file/record-injection attack.
%Furthermore, \framework offers a flexible key management scheme where revoking users does not require regeneration of keys and re-encryption of the data.

As future work, first we will do our performance analysis by deploying the scheme in the real multi-cloud setting.
Second, we will try to address the limitations of \framework.
Specifically, \framework protects the search, access, and size patterns from the CSPs.
However, it suffers from the collusion attack among CSPs.
In \framework, the SSS knows the search result for each query, and the other two knows how the records are shuffled and re-randomised.
If the SSS colludes with the IWS or RSS, they could learn the search and access patterns.
We will also consider the techniques to defend the collusion attack among CSPs.
Moreover, in this work, we assume all the CSPs are honest.
Yet, in order to learn more useful information, the compromised CSPs might not behave honestly as assumed in the security analysis.
For instance, the SSS might not search all the records indexed by $IL$, and the RSS might not shuffle the records properly.
In the future, we will give a mechanism to detect if the CSPs honestly follow the designated protocols.


==> PMcDb_arXiv/sections/details.tex <==
\section{Solution details}
\label{sec:MCDB-details}
%
\begin{table}[htp]
\scriptsize
%\small
\centering
\caption{Data representation in \framework}
\subtable[\emph{Staff}]
{
\label{Tbl:mcdb-staff}
\begin{tabular}{|c|c|}\hline
\textbf{Name} & \textbf{Age} \\\hline
Alice & 27    \\\hline
Anna  & 30    \\\hline
Bob   & 27    \\\hline
Bill  & 25    \\\hline
Bob   & 33    \\\hline
%Baker & 25    \\\hline
\end{tabular}
}
%\hspace*{3mm}
\subtable[GDB on the IWS]
{
\label{Tbl:mcdb-engid}
\begin{tabular}{|c|c|c|c|}\hline
 \textbf{GID}    & \textbf{IL}        &$(\bm{E}, \tau)^*$         \\ \hline
 $(1, g_{1})$    & $\{1, 2\}$         & $(\{Alice, Anna\}, 1)^*$  \\\hline
 $(1, g_{2})$    & $\{3, 4, 5, 6\}$   & $(\{Bob, Bill\}, 2)^*$    \\\hline
 $(2, g'_{1})$   & $\{1, 3, 4, 6\}$   & $(\{25, 27\}, 2)^*$       \\\hline
 $(2, g'_{2})$   & $\{2, 5\}$         & $(\{30, 33\}, 1)^*$       \\\hline
\end{tabular}
}
%
\subtable[NDB on the IWS]
{
\label{Tbl:mcdb-nonceI}
\begin{tabular}{|c|c|c|}\hline
\textbf{id} &$\bm{seed}$ & $\bm{nonce}$ \\ \hline
1 & $seed_{1}$  & $\bm{n_1}$ \\\hline
2 & $seed_{2}$  & $\bm{n_2}$ \\\hline
3 & $seed_{3}$  & $\bm{n_3}$ \\\hline
4 & $seed_{4}$  & $\bm{n_4}$ \\\hline
5 & $seed_{5}$  & $\bm{n_5}$ \\\hline
6 & $seed_{6}$  & $\bm{n_6}$ \\\hline
%7 & $seed_{7}$  \\\hline
%8 & $seed_{8}$  \\\hline
%4 & $seed_{4}$  & $1$\\\hline
\end{tabular}
}
%
\subtable[EDB on the SSS]
{
\label{Tbl:mcdb-enstaff}
\begin{tabular}{|c|c|c|c|c|}\hline
\textbf{ID} & \textbf{1}  & \textbf{2} & \textbf{Tag} \\\hline
1  & $SE(Alice)$  & $SE(27)$  & $tag_1$  \\\hline
2  & $SE(Anna)$   & $SE(30)$  & $tag_2$  \\\hline
3  & $SE(Bob)$    & $SE(27)$  & $tag_3$  \\\hline
4  & $SE(Bill)$   & $SE(25)$  & $tag_4$  \\\hline
5  & $SE(Bob)$    & $SE(33)$  & $tag_5$  \\\hline
%6  & $SE(Baker)$  & $SE(25)$  & $tag_6$  \\\hline
6  & $SE(Bill)$   & $SE(25)$  & $tag_6$   \\\hline
%8  & $SE(Baker)$  & $SE(27)$  & $tag_8$   \\\hline
\end{tabular}
}
\label{Tbl:mcdb-store}

 \subref{Tbl:mcdb-staff} A sample \emph{Staff} table.
 \subref{Tbl:mcdb-engid} GDB, the group information, is stored on the IWS.
 \subref{Tbl:mcdb-nonceI} NDB contains the seeds used to generate nonces.
 It might contain the nonces directly.
 NDB is also stored on the IWS.
 %For each record $rcd_i$, the IWS stores a seed $seed_{i}$.
 \subref{Tbl:mcdb-enstaff} EDB, the encrypted \emph{Staff} table, is stored on the SSS.
 Each encrypted data element $SE(e_f)=Enc_{s_1}(e_f)\oplus n_f$.
 Each record has a tag, enabling users to distinguish dummy and real records.
 In this example, the last record in Table~\subref{Tbl:mcdb-enstaff} is dummy.
 The RSS does not store any data.
\end{table}
%
\begin{algorithm}[tp]
\scriptsize
%\small
\caption{$Setup(k, DB)$}
\label{alg:mcdb-setup}
\begin{algorithmic}[1]
\STATE \underline{Admin: $KeyGen$}
\STATE $s_1, s_2 \lt \{0, 1\}^k$
~\\~
\STATE $GDB \lt \emptyset$, $EDB \lt \emptyset$, $NDB \lt \emptyset$
\STATE \underline{Admin: $GroupGen$} \label{code:setup-grpgen-be}
\FOR{each field $f$}
    \STATE Collect $U_f$ and $\{O(e)\}_{e \in U_f}$, and compute $\Psi_f=\{g \lt GE_{s_1}(e)\}_{e \in U_f}$
    \FOR{each $g \in \Psi_f$}
        \STATE $IL_{f, g} \lt \emptyset$, $\bm{E}_{f, g} \lt \{e\}_{e\in U_f \& GE_{s_1}(e)=g}$  \label{code:setup-grpgen-e}
        \STATE $\tau_{f, g} \lt \max\{|O(e)|\}_{e \in \bm{E}_{f, g}}$ \label{code:setup-grpgen-t}
        \STATE $(\bm{E}_{f, g}, \tau)^* \lt ENC_{s_1}(\bm{E}_{f, g}, \tau)$
            \label{code:setup-gdb}
        \STATE $GDB(f, g) \lt (IL_{f, g}, (\bm{E}_{f, g}, \tau_{f, g})^*)$
    \ENDFOR

\ENDFOR \label{code:setup-grpgen-end}

~\\~
\STATE \underline{Admin: DummyGen}\label{code:setup-dummygen-be}
\FOR{each field $f$}
    \STATE $\Sigma_f \lt \Sigma_{g \in \Psi_f}\Sigma_{e \in \bm{E}_{f, g}} (\tau_{f, g} - O(e))$
\ENDFOR
\STATE $\Sigma_{max} \lt \max\{\Sigma_1, \ldots, \Sigma_F\}$
\STATE Add $\Sigma_{max}$ dummy records with values $(NULL, \ldots, NULL)$ into $DB$
\FOR {each field $f$}
    \FOR {each $e \in U_f$}
        \STATE Assign $e$ to $\tau_{f, GE_{s_1}(e)}-O(e)$ dummy records in field $f$
    \ENDFOR
\ENDFOR
\STATE Mark real and dummy records with $flag=1$ and $flag=0$, respectively
\STATE Shuffle $DB$ \label{code:setup-dummygen-end}

~\\~
\STATE \underline{Admin: DBEnc} \label{code:setup-DBenc-be}
\STATE $id \lt 0$
\FOR{each $rcd \in DB$}
    \STATE $(Ercd, seed, \bm{n}, Grcd)\lt RcdEnc(rcd, flag)$
    \STATE $EDB(id) \lt Ercd$, $NDB(id) \lt (seed, \bm{n})$
    \FOR{each $g_f \in Grcd$}
        \STATE $IL_{f, g} \lt IL_{f, g} \cup id$  \label{code:setup-DBenc-IL}
    \ENDFOR
    \STATE $id++$  \label{code:setup-DBenc-end}
\ENDFOR
\end{algorithmic}
\end{algorithm}
%

In this section, we give the details for setting up, searching, and updating the database.

\subsection{Setup}
\label{subsec:boot}
The system is set up by the admin by generating the secret keys $s_1$ and $s_2$ based on the security parameter $k$.
$s_1$ is only known to users and is used to protect queries and records from CSPs.
$s_2$ is generated for saving storage, and it is known to both the user and IWS and is used to generate nonces for record and query encryption.
%
The admin also defines the cryptographic primitives used in \framework.

We assume the initial database $DB$ is not empty.
The admin bootstraps $DB$ with Algorithm \ref{alg:mcdb-setup}, $Setup(k, DB) \rt (EDB, GDB, NDB)$.
Roughly speaking, the admin divides the records into groups (Lines \ref{code:setup-grpgen-be}-\ref{code:setup-grpgen-end}), pads the elements in the same group into the same occurrence by generating dummy records (Lines \ref{code:setup-dummygen-be}-\ref{code:setup-dummygen-end}), and encrypts each record (Lines \ref{code:setup-DBenc-be}-\ref{code:setup-DBenc-end}).
The details of each operation are given below.

\paragraph{Group Generation}
%Given $DB$, the admin first divides the data into groups and pads the elements in the same group into the same occurrence with dummy records.
As mentioned, inserting dummy records is necessary to protect the size and search patterns, and grouping the data aims at reducing the number of required dummy records.

Indeed, dividing the data into groups could also reduce the number of records to be searched.
Only padding the data in the same group into the same occurrence could result in the leakage of group information.
Particularly, the SSS can learn if records and queries are in the same group from the size pattern.
Considering the group information will be inevitably leaked after executing queries, \framework allows the SSS to know the group information in advance, and only search a group of records for each query rather than the whole database.
By doing so, the query can be processed more efficiently without leaking additional information.
Yet, in this case, the SSS needs to know which group of records should be searched for each query.
Considering the SSS only gets encrypted records and queries, the group should be determined by the admin and users.
To avoid putting heavy storage overhead on users, \framework divides data into groups with a Pseudo-Random Function (PRF) $GE: \{0, 1\}^* \times \{0, 1\}^k \rightarrow \{0, 1\}^*$.
The elements in field $f$ ($1\leq f \leq F$) with the same $g \leftarrow GE_{s_1}(e)$ value are in the same group, and $(f, g)$ is the group identifier.
In this way, the admin and users can easily know the group identifiers of records and queries just by performing $GE$.

The implementation of $GE$ function affects the security level of the search pattern.
Let $\lambda$ stand for the number of distinct elements contained in a group.
Since the elements in the same group will have the same occurrence, the queries involving those elements (defined as \emph{the queries in the same group}) will match the same number of records.
Then, the adversary cannot tell their search patterns from their size patterns.
Formally, for any two queries matching the same number of records, the probability they involve the same keyword is $\frac{1}{\lambda}$.
Thus, $\lambda$ also represents the security level of the search pattern.
Given $\lambda$, the implementation of $GE$ should ensure each group contains at least $\lambda$ distinct elements.
For instance, the admin could generate the group identifier of $e$ by computing $LSB_b(H_{s_1}(e))$, where $LSB_b$ gets the least significant $b$ bits of its input.
To ensure each group contains at least $\lambda$ distinct elements, $b$ can be smaller.

The details of grouping $DB$ are shown in Lines \ref{code:setup-grpgen-be}-\ref{code:setup-grpgen-end} of Algorithm \ref{alg:mcdb-setup}.
Formally, we define group $(f, g)$ as $(IL_{f, g}, \bm{E}_{f, g}, \tau_{f, g})$, where $IL_{f, g}$ stores the identifiers of the records in this group (Line \ref{code:setup-DBenc-IL}), $\bm{E}_{f, g}$ is the set of distinct elements in this group (Line \ref{code:setup-grpgen-e}), and $\tau_{f, g}=\max\{O(e) | e \in \bm{E}_{f, g}\}$ is the occurrence threshold for padding (Line \ref{code:setup-grpgen-t}).
Since the group information will be stored in the CSP, $(\bm{E}_{f, g}, \tau_{f, g})$ is encrypted into $(\bm{E}_{f, g}, \tau_{f, g})^*$ with $s_1$ and a semantically secure symmetric encryption primitive $ENC: \{0, 1\}^* \times \{0, 1\}^k \rt \{0, 1\}^*$.
$(\bm{E}_{f, g}, \tau_{f, g})^*$ is necessary for insert queries (The details are given in Section~\ref{subsec:update}).

Note that if the initial database is empty, the admin can pre-define a possible $U_f$ for each field and group its elements in the same way.
In this case, $IL=\emptyset$ and $\tau=0$ for each group after the bootstrapping.

\paragraph{Dummy Records Generation}
Once the groups are determined, the next step is to generate dummy records.
The details for generating dummy records are given in Lines \ref{code:setup-dummygen-be}-\ref{code:setup-dummygen-end}, Algorithm \ref{alg:mcdb-setup}.
Specifically, the admin first needs to know how many dummy records are required for the padding.
Since the admin will pad the occurrence of each element in $\bm{E}_{f, g}$ into $\tau_{f, g}$, $\tau_{f, g}-O(e)$ dummy records are required for each $e \in \bm{E}_{f, g}$.
%for the number of required dummy records for this group is $\sum_{e \in \bm{E}_{f, g}}(\tau_{f, g}-O(e))$.

Assume there are $M$ groups in field $f$, then $\Sigma_f=\sum_{i=1}^{M}\sum_{e \in \bm{E}_{f, g^i}}(\tau_{f, g^i}-O(e))$ dummy records are required totally for padding field $f$.
For the database with multiple fields, different fields might require different numbers of dummy records.
Assume $\Sigma_{max}=\max\{\Sigma_1, \ldots, \Sigma_F\}$.
To ensure all fields can be padded properly, $\Sigma_{max}$ dummy records are required.
Whereas, $\Delta_f=\Sigma_{max} - \Sigma_f$ dummy records will be redundant for field $f$.
%The issue is what the admin can assign to field $f$ for the $\Delta_f$ redundant records. If the admin keeps them unassigned, the CSP can tell the incomplete records are dummy. On the contrary, if the admin assigns them also with the elements in $U_f$, it is hard to ensure the elements in each group still have the same occurrence.
The admin assigns them a meaningless string, such as `NULL', in field $f$.
After encryption, `NULL' will be indistinguishable from other elements.
Thus, the CSP cannot distinguish between real and dummy records.
%Moreover, `NULL' does not affect the occurrence of other elements.
Note that users and the admin can search the records with `NULL'.

In this work, we do not consider the query with conjunctive predicates, so we do not consider to pad the element pairs also into the same occurrence.

After padding, each record $rcd$ is appended with a $flag$ to mark if it is real or dummy.
Specifically, $flag=1$ when $rcd$ is real, otherwise $flag=0$.
The admin also shuffles the dummy and real records.

\paragraph{Record Encryption}
%
\begin{algorithm}[tp]
\scriptsize
%\small
\caption{$RcdEnc(rcd, flag)$}
\label{alg:mcdb-enc}
\begin{algorithmic}[1]
   \STATE $seed \stackrel{\$}{\leftarrow} \{0,1\}^{|seed|}$
   \STATE $\bm{n} \leftarrow \Gamma_{s_2} (seed)$, where $\bm{n}=\ldots \| n_f \| \ldots \| n_{F+1}$, $|n_f|=|e|$ and $|n_{F+1}|=|H|+|e|$ \label{code:mcdb-enc-seed}
    \FOR {each element $e_f \in rcd$}
        \STATE $g_f \lt GE_{s_1}(e_f)$  \label{code:mcdb-enc-gid}
        %\STATE $\sigma \lt Enc_{s_1}(e_f)$
        \STATE $e^*_f \lt  Enc_{s_1}(e_f) \oplus n_f$  \label{code:mcdb-enc-se}
    \ENDFOR
    \IF {$flag=1$}
        %\STATE $n_{F+1} \lt n_{[f|e|+1, f|e|+2k]}$
        \STATE $S \stackrel{\$}{\leftarrow} \{0,1\}^{|e|}$
        \STATE $tag \leftarrow (H_{s_1}(S)||S )\oplus n_{F+1}$ \label{code:mcdb-enc-tag-re}
    \ELSE
        \STATE $tag \stackrel{\$}{\leftarrow} \{0,1\}^{|H|+|e|}$ \label{code:mcdb-enc-tag-du}
    \ENDIF
\RETURN $Ercd=(e^*_1, \ldots, e^*_F, tag)$, $(seed, \bm{n})$, and $Grcd=(g_1, \ldots, g_F)$
\end{algorithmic}
\end{algorithm}
%
The admin encrypts each record before uploading them to the SSS.
The details of record encryption are provided in Algorithm~\ref{alg:mcdb-enc}, $RcdEnc (rcd, flag) \rightarrow (Ercd, seed, \bm{n}, Grcd)$.

To ensure the dummy records could match queries, they are encrypted in the same way as real ones.
%Specifically, $RcdEnc$ takes the record $rcd=(e_1, ..., e_F)$ and the $flag$ as the inputs, and outputs the encrypted record $Ercd$, a $seed$, a nonce $\bm{n}$, and the group information $Grcd$.
Specifically, first the admin generates a random string as a $seed$ for generating a longer nonce $\bm{n}$ with a Pseudo-Random Generator (PRG) $\Gamma: \{0, 1\}^{|seed|} \times \{0, 1\}^{k} \rightarrow \{0, 1\}^{*}$ (Line~\ref{code:mcdb-enc-seed}, Algorithm~\ref{alg:mcdb-enc}).
%The user does not have to remember the seed $seed$ or the nonce $\bm{n}$; this is the job of the IWS.
Second, the admin generates $g_f$ for each $e_f \in rcd$ by computing $GE_{s_1}(e_f)$ (Line \ref{code:mcdb-enc-gid}).
Moreover, $e_f$ is encrypted by computing $SE(e_f): e^*_f \leftarrow Enc_{s_1}(e_f) \oplus n_f$ (Line~\ref{code:mcdb-enc-se}), where $Enc:\{0,1\}^* \times \{0,1\}^k \rightarrow \{0,1\}^* $ is a deterministic symmetric encryption primitive, such as AES-ECB.
Using $n_f$, on the one hand, ensures the semantically secure of $e^*_f$.
On the other hand, it ensures the forward and backward privacy of \framework (as explained in Section \ref{subsec:shuffle}).
$e^*_f$ will be used for encrypted search and data retrieval.

The dummy records are meaningless items, and the user does not need to decrypt returned dummy records.
Thus, we need a way to filter dummy records for users.
Considering the CSPs are untrusted, we cannot mark the real and dummy records in cleartext.
Instead, we use a keyed hash value to achieve that.
Specifically, as shown in Lines~\ref{code:mcdb-enc-tag-re} and \ref{code:mcdb-enc-tag-du}, a tag $tag$ is generated using a keyed hash function $H: \{0,1\}^* \times \{0,1\}^k \rightarrow \{0,1\}^*$ and the secret key $s_1$ if the record is real, otherwise $tag$ is a random bit string.
With the secret key $s_1$, the dummy records can be efficiently filtered out by users before decrypting the search result by checking if:
\begin{align}\label{eq:check1}\notag
  tag_{l} \stackrel{?}{=}& H_{s_1}(tag_{r}), \text{ where } tag_{l}||tag_{r} = tag \oplus n_{F+1}
\end{align}

%\paragraph{Data Representation}
Once all the real and dummy records are encrypted, the admin uploads the auxiliary information, \ie the set of group information $GDB$ and the set of nonce information $NDB$, to the IWS, and uploads encrypted records $EDB$ to the SSS.
%Table \ref{Tbl:mcdb-store} provides an example of $GDB$, $NDB$, and $EDB$ for the \emph{Staff} table shown in cleartext in Table \ref{Tbl:mcdb-staff}.
%In our example, the \emph{Staff} table has 2 fields and contains 5 records. For each field, the 5 records are divided into 2 groups.
$GDB$ contains $(IL, (\bm{E}, \tau)^*)$ for each group. %(shown in Table \ref{Tbl:mcdb-engid})
%In the example, for \emph{name} field, group $g_{1, 1}$ contains $\{Alice, Anna\}$, and both $Alice$ and $Anna$ only occurs once in the database.
$NDB$ contains a $(seed, \bm{n})$ pair for each record stored in $EDB$. %(shown in Table \ref{Tbl:mcdb-nonceI})
To reduce the storage overhead on the IWS, $NDB$ could also just store the seed and recover $\bm{n}$ by computing $\Gamma_{s_2}(seed)$ when required.
Whereas, saving the $(seed, \bm{n})$ pairs reduces the computation overhead on the IWS.
In the rest of this article, we assume NDB contains $(seed, \bm{n})$ pairs.
$EDB$ contains the encrypted record $Ercd$. %(shown in Table \ref{Tbl:mcdb-enstaff})
Note that to ensure the correctness of the search functionality, it is necessary to store the encrypted records and their respective $(seed, \bm{n})$ pairs in the same order in $EDB$ and $NDB$ (the search operation is explained in Section \ref{subsec:mcdb-select}).
In Table~\ref{Tbl:mcdb-store}, we take the \emph{Staff} table (\ie Table \ref{Tbl:mcdb-staff}) as an example and show the details stored in $GDB$, $NDB$, and $EDB$ in Tables~\ref{Tbl:mcdb-engid},~\ref{Tbl:mcdb-nonceI}, and~\ref{Tbl:mcdb-enstaff}, respectively.

%In addition to the database fields (\ie \emph{Name} and \emph{Age}), $EDB$ also contains the tag field for $tag$. $EDB$ contains one extra record with $id$ 6: it is a dummy record generated by the admin.

%The field names in Tables \ref{Tbl:mcdb-enstaff} (as well as in queries) are encrypted with $H_{s_1}$.
%
%\footnote{$gid_a \leftarrow f_s_1(Alice)$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%       S E L E C T     %%%%%%%%%%%%%%%

\subsection{Select Query}
\label{subsec:mcdb-select}
%
\begin{algorithm}[htp]
\scriptsize
%\small
\caption{Query$(Q)$}
\label{alg:macdb-search}
\begin{algorithmic}[1]
\STATE \underline{User: QueryEnc$(Q)$}  \label{code:mcdb-query-user-be}
    %\STATE $\sigma \leftarrow H_{s_1}(Q.e) $
    \STATE $g \leftarrow GE_{s_1}( Q.e )$ \label{code:mcdb-query-user-gid}
    \STATE $EQ.type \lt Q.type$, $EQ.f \lt Q.f$
    \STATE $\eta \stackrel{\$}{\lt} \{0,1\}^{|e|}$
    %\STATE $\sigma \lt Enc_{s_1}(Q.e)$
    \STATE $EQ.e^*  \lt Enc_{s_1}(Q.e) \oplus \eta$  \label{code:mcdb-query-se}
    \STATE Send $EQ=(type, f, e^*)$ to the SSS
    \STATE Send $(EQ.f, \eta, g)$ to the IWS \label{code:mcdb-query-user-end}
%\end{algorithmic}
%
~\\~

%\begin{algorithmic}[1]
\STATE \underline{IWS: $NonceBlind(EQ.f, \eta, g)$} \label{code:mcdb-query-IWS-be}
    \STATE $EN \leftarrow \emptyset$
    \STATE $IL \leftarrow GDB(EQ.f, g)$ \COMMENT{If $(EQ.f, g) \notin GDB$, return $IL$ of the  closest group(s).}\label{code:mcdb-query-IL}
    \FOR {each $id \in IL$ }
        \STATE  $(seed, \bm{n}) \leftarrow NDB(id)$, where $\bm{n}= \ldots ||n_{EQ.f}|| \ldots$ and $|n_{EQ.f}|=|\eta|$
                \label{code:mcdb-query-get-nonce}
        \STATE  $w \lt H'(n_{EQ.f} \oplus \eta)$
        \STATE  $t \lt \eta \oplus seed$
        \STATE  $EN(id) \leftarrow (w, t)$ \label{code:mcdb-query-enc-nonce}
    \ENDFOR
    \STATE Send $IL=(id, \ldots)$ and the encrypted nonce set $EN=((w, t), \ldots)$ to the SSS   \label{code:mcdb-query-IWS-end}

~\\
%\begin{algorithmic}[1]
\STATE \underline{SSS: $Search(EQ, EN, IL)$}   \label{code:mcdb-query-SSS-be}
    \STATE $SR \leftarrow \emptyset$
    \FOR {each $id \in IL$}
        \IF {$H'(EDB(id, EQ.f) \oplus EQ.e^*) = EN(id).w$ }  \label{code:mcdb-query-checke}
             \STATE $SR \leftarrow SR \cup (EDB(id), EN(id).t)$ \label{code:mcdb-query-sr}
        \ENDIF
    \ENDFOR
    \STATE Send the search result $SR$ to the user \label{code:mcdb-query-SSS-end}

~\\
\STATE \underline{User: RcdDec$(SR, \eta)$} \label{code:mcdb-query-dec-be}
\FOR{each $(Ercd, t) \in SR$}
    \STATE  $\bm{n} \leftarrow \Gamma_{s_2} (t \oplus \eta)$ \label{code:mcdb-query-dec-seed}
    \STATE  $(Enc_{s_1}(rcd), tag) \leftarrow Ercd \oplus \bm{n}$
    \STATE $tag_{l} || tag_{r} \lt tag$, where $|tag_r|=|e|$
    \IF{$tag_{l} = H_{s_1}(tag_{r})$} \label{code:mcdb-query-ducheck}
        \STATE  $rcd \leftarrow Enc^{-1}_{s_1} (Enc_{s_1}(rcd))$ \label{code:mcdb-query-dec}
    \ENDIF
\ENDFOR \label{code:mcdb-query-dec-end}
%\end{multicols}
\end{algorithmic}
\end{algorithm}
%
In this work, we focus on the simple query which only has one single equality predicate.
The complex queries with multiple predicates can be performed by issuing multiple simple queries and combing their results on the user side.
To support range queries, the technique used in \cite{Asghar:Espoon:IRC13} can be adopted. %, where numbers are converted into several bags of bit strings, and an inequality over a number is converted into several equalities over bit strings.

For performing a select query, \framework requires the cooperation between the IWS and SSS.
The details of the steps performed by the user, IWS, and SSS are shown in Algorithm~\ref{alg:macdb-search}, $Query(Q) \rightarrow SR$, which consists of 4 components: $QueryEnc$, $NonceBlind$, $Search$, $RcdDec$.

\paragraph{\bm{$QueryEnc(Q)\rightarrow (EQ, \eta, g)$}}
First, the user encrypts the query $Q=(type, f, e)$ using $QueryEnc$ (Lines \ref{code:mcdb-query-user-be} - \ref{code:mcdb-query-user-end}, Algorithm \ref{alg:macdb-search}).
Specifically, to determine the group to be searched, the user first generates $g$ (Line \ref{code:mcdb-query-user-gid}).
We do not aim at protecting the query type and searched field from CSPs.
Thus, the user does not encrypt $Q.type$ and $Q.f$.
%The searched field $Q.f$ is hashed with $s_1$.
The interested keyword $Q.e$ is encrypted into $EQ.e^*$ by computing $Enc_{s_1}(Q.e)\oplus \eta$ (Line \ref{code:mcdb-query-se}).
The nonce $\eta$ ensures that $EQ.e^*$ is semantically secure.
Finally, the user sends $EQ=(type, f, e^*)$ to the SSS and sends $(EQ.f$, $\eta$, $g)$ to the IWS.

\paragraph{$\bm{NonceBlind(EQ.f, \eta, g)\rightarrow (IL, EN)}$}
Second, the IWS provides $IL$ and witnesses $EN$ of group $(EQ.f, g)$ to the SSS by running $NonceBlind$ (Line \ref{code:mcdb-query-IWS-be} - \ref{code:mcdb-query-IWS-end}).
Specifically, for each $id \in IL$, the IWS generates $EN(id)=(w, t)$ (Lines~\ref{code:mcdb-query-get-nonce}-\ref{code:mcdb-query-enc-nonce}),
where $w=H'(n_{EQ.f} \oplus \eta)$ will be used by the SSS to find the matching records, and $t= \eta \oplus seed$ will be used by the user to decrypt the result.
Here $H': \{0, 1\}^* \rt \{0, 1\}^k$ is a hash function.
Note that when $(EQ.f, g)$ is not contained in $GDB$, $IL$ of the \emph{closest} group(s) will be used, \ie the group in field $EQ.f$ whose identifier has the most common bits with $g$\footnote{This can be obtained by comparing the hamming weight of $g' \oplus g$ for all $(EQ.f, g') \in GDB$.}.

\paragraph{$\bm{Search(EQ, IL, EN)\rightarrow SR}$}
Third, the SSS traverses the records indexed by $IL$ and finds the records matching $EQ$ with the assistance of $EN$ (Lines \ref{code:mcdb-query-SSS-be} - \ref{code:mcdb-query-SSS-end}).
Specifically, for each record indexed by $IL$, the SSS checks if $H'(EDB(id, EQ.f) \oplus EQ.e^*) \stackrel{?}{=} EN(id).w$ (Line \ref{code:mcdb-query-checke}).
More specifically, the operation is:
%
\begin{equation}\notag
 H'(Enc_{s_1}(e_{EQ.f})\oplus n_{EQ.f}  \oplus Enc_{s_1}(Q.e) \oplus \eta ) \stackrel{?}{=} H'(n_{EQ.f} \oplus \eta)
\end{equation}
%
It is clear that only when $Q.e=e_{EQ.f}$ there is a match.
The SSS sends each matched record $EDB(id)$ and its corresponding $EN(id).t$ to the user as the search result $SR$, \ie $EDB(EQ)$.


\paragraph{\bm{$RcdDec(SR) \rightarrow rcds$}}
To decrypt an encrypted record $Ercd$, both the secret key $s_1$ and nonce $\bm{n}$ are required.
The nonce $\bm{n}$ can be recovered from the returned $t$.
Only the user issuing the query knows $\eta$ and is able to recover $\bm{n}$ by computing $\Gamma_{s_2}(t \oplus \eta)$ (Line \ref{code:mcdb-query-dec-seed}).
With $\bm{n}$, the user can check if each returned record is real or dummy (Line \ref{code:mcdb-query-ducheck}), and decrypt each real record by computing
$Enc^{-1}_{s_1}(Ercd \oplus \bm{n})$ (Line \ref{code:mcdb-query-dec}), where $Enc^{-1}$ is the inverse of $Enc$.

\subsection{Shuffling and Re-randomisation}
\label{subsec:shuffle}
%
\begin{algorithm}
%\small
\scriptsize
\caption{$Shuffle(IL, Ercds)$}
\label{alg:mcdb-shuffle}
\begin{algorithmic}[1]
\STATE \underline{IWS: $PreShuffle(IL)$} \label{code:mcdb-preshuffle-be}
    \STATE $IL' \leftarrow \pi (IL)$
    \STATE Shuffle the $(seed, \bm{n})$ pairs indexed by $IL$ based on $IL'$
    \STATE Update the indices of affected groups in $GDB$ \label{code:mcdb-shuffle-update-groups}
    \FOR {each $id \in IL'$} \label{code:mcdb-shuffle-begin}
        \STATE $seed \stackrel{\$}{\leftarrow} \{0, 1\}^{|seed|}$ \label{code:mcdb-seed'}
        \STATE $\bm{n'} \leftarrow  \Gamma_{s_2}(seed)$ \label{code:mcdb-gn'}
        \STATE $NN(id) \leftarrow NDB(id).\bm{n} \oplus \bm{n'}$ \label{code:mcdb-nn}
        \STATE $NDB(id) \leftarrow (seed, \bm{n'})$ \label{code:mcdb-n'}
    \ENDFOR
    \STATE Send $(IL', NN)$ to the RSS. \label{code:mcdb-preshuffle-end}

~\\~
\STATE{\underline{RSS: $Shuffle(Ercds, IL', NN)$}}
    \STATE Shuffle $Ercds$ based on $IL'$
    \FOR {each $id \in IL'$}
        \STATE $Ercds(id) \leftarrow Ercds(id) \oplus NN(id) $   \label{code:mcdb-shuffle-reenc}
    \ENDFOR
    \STATE Send $Ercds$ to the SSS.
\end{algorithmic}
%\end{multicols}
\end{algorithm}
%

To protect the access pattern and ensure the forward and backward privacy, \framework shuffles and re-randomises searched records after executing each query, and this procedure is performed by the IWS and RSS.
The details are shown in Algorithm \ref{alg:mcdb-shuffle}, consisting of $PreShuffle$ and $Shuffle$.
%After each insert, select and delete query, the SSS should send the records to the IWS for shuffling.

\paragraph{$\bm{PreShuffle(IL) \rightarrow (IL', NN)}$}
%To make the records untraceable for the SSS, it is necessary to re-randomise the searched records.
In \framework, the searched records are re-randomised by renewing the nonces.
Recall that $SE$ encryption is semantically secure due to the nonce.
However, the IWS stores the nonces.
If the IWS has access to encrypted records, it could observe deterministically encrypted records by removing the nonces.
To void leakage, \framework does not allow the IWS to access any records and involves the RSS to shuffle and re-randomise the records.

Yet, the IWS still needs to shuffle $NDB$ and generate new nonces for the re-randomisation by executing $PreShuffle$.
Specifically, as shown in Algorithm \ref{alg:mcdb-shuffle}, Lines \ref{code:mcdb-preshuffle-be}-\ref{code:mcdb-preshuffle-end}, the IWS first shuffles the $id$s in $IL$ with a Pseudo-Random Permutation (PRP) $\pi$ and gets the re-ordered indices list $IL'$.
In our implementation, we leverage the modern version of the Fisher-Yates shuffle algorithm \cite{Knuth73}, where from the first $id$ to the last one, each $id$ in $IL$ is exchanged with a random $id$ storing behind it.
After that, the IWS shuffles $(seed, \bm{n})$ pairs based on $IL'$.
Note that the shuffling operation affects the list of indices of the groups in other fields.
Thus, the IWS also needs to update the index lists of other groups accordingly (Line \ref{code:mcdb-shuffle-update-groups}).
For re-randomising records, the IWS samples a new seed and generates a new nonce $\bm{n'}$.
To ensure the records will be blinded with the respective new nonces stored in $NDB$ after shuffling and re-randomising, the IWS generates $NN=(\bm{n}\oplus\bm{n'}, \ldots)$ for RSS (Line \ref{code:mcdb-nn}).
Afterwards, IWS updates the seed and nonce stored in $NDB(id)$ with the new values.
Finally, $(IL', NN)$ is sent to the RSS.

%Note that when the database only supports searching over one field, the elements in other fields can be encrypted entirely with semantically secure primitive . In this case, the IWS cannot get any co-occurrence even if it has access to encrypted records, and the following shuffle algorithm can be performed on the IWS.

\paragraph{$\bm{Shuffle(Ercds, IL', NN) \rightarrow Ercds}$}
After searching, the SSS sends the searched records $Ercds$ to the RSS.
Given $IL'$ and $NN$, the RSS starts to shuffle and re-randomise $Ercds$.
Specifically, the RSS first shuffles $Ercds$ based on $IL'$, and then re-randomises each record by computing $Ercds(id) \oplus NN(id)$ (Line \ref{code:mcdb-shuffle-reenc}).
In details, the operation is:
%
\begin{equation}\notag
 (Enc_{s_1}(rcd_{id})\oplus \bm{n})  \oplus (\bm{n'} \oplus \bm{n}) = Enc_{s_1}(rcd_{id})\oplus \bm{n'}
\end{equation}
%
That is, $Ercds(id)$ is blinded with the latest nonce stored in $NDB(id)$.
Finally, the re-randomised and shuffled records $Ercds$ are sent back to the SSS.

By using a new set of seeds for the re-randomisation, \framework achieves both forward and backward privacy.
If the SSS tries to execute an old query individually, it will not be able to match any records without the new witness $w$, which can only be generated by the IWS with new nonces.
Similarly, the SSS cannot learn if deleted records match new queries.


\subsection{User Revocation}
\label{sec:revoke}
\framework supports flexible multi-user access in a way that the issued queries and search results of one user are protected from all the other entities. Moreover, revoking users do not require key regeneration and data re-encryption even when one of the CSPs colludes with revoked users.

As mentioned in Section \ref{subsec:mcdb-select}, for filtering dummy records and recovering returned real records, both $s_1$ and the nonce are required.
After shuffling, the nonce is only known to the IWS.
Thus, without the assistance of the IWS and SSS, the user is unable to recover records only with $s_1$.
Therefore, for user revocation, we just need to manage a revoked user list at the IWS as well as at the SSS.
Once a user is revoked, the admin informs the IWS and SSS to add this user into their revoked user lists.
When receiving a query, the IWS and the SSS will first check if the user has been revoked.
If yes, they will reject the query.
In case revoked users collude with either the SSS or IWS, they cannot get the search results, since such operation requires the cooperation of both the user issuing the query, IWS, and SSS.


\subsection{Database Updating}
\label{subsec:update}
%
\begin{algorithm}
%\small
\scriptsize
\caption{$Insert(rcd)$}
\label{alg:mcdb-insert}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\STATE \underline{$User(rcd)$}:
%\STATE $INS_{IWS} \lt \emptyset$, $INS_{SSS} \lt \emptyset$
\STATE $(Ercd, seed, \bm{n}, Grcd) \lt RcdEnc(rcd, 1)$ \label{code:mcdb-insert-user-enc}
\STATE $INS_{IWS} \lt (seed, \bm{n}, Grcd)$, $INS_{SSS} \lt  Ercd$
\FOR {each $g_f \in Grcd$}   \label{code:mcdb-insert-user-be}
    \STATE $(\bm{E}_{f, g_f}, \tau_{f, g_f})^* \lt GDB(f, g_f)$\COMMENT{If $(f, g_f) \notin GDB$, $g_f \lt g_f'$, where $(f, g_f')$ is the closet group of $(f, g_f)$.}
    \STATE $(\bm{E}_{f, g_f}, \tau_{f, g_f}) \lt ENC^{-1}_{s_1}((\bm{E}_{f, g_f}, \tau_{f, g_f})^*)$ \label{code:mcdb-insert-user-ef}
\ENDFOR
\FOR{each $e_f \in rcd$}  \label{code:mcdb-insert-gendum-be}
    \IF{$e_f \in \bm{E}_{f, g_f}$}
        \STATE $\gamma_{f} \lt |\bm{E}_{f, g_f}| -1 $
    \ELSE
        \STATE $\gamma_{f} \lt \tau_{f, g_f} -1 $
    \ENDIF
\ENDFOR
\STATE $W=\max\{\gamma_{f}\}_{1 \leq f \leq F}$ \label{code:mcdb-insert-encdum-be}
\STATE Generate $W$ dummy records with values $(NULL, \ldots, NULL)$
\FOR{each $e_f \in rcd$}
    \IF{$e_f \in \bm{E}_{f, g_f}$}
        \STATE Assign $\bm{E}_{f, g_f} \setminus e_f$ to $\gamma_f$ dummy records in field $f$
        \STATE $\tau_{f, g_f} ++$
    \ELSE
        \STATE Assign $e_f$ to $\gamma_f$ dummy records in field $f$
        \STATE $\bm{E}_{f, g_f} \lt \bm{E}_{f, g_f} \cup e_f$
    \ENDIF
    \STATE $(\bm{E}_{f, g_f}, \tau_{f, g_f})^* \lt ENC_{s_1}(\bm{E}_{f, g_f}, \tau_{f, g_f})$  \label{code:mcdb-insert-gendum-end}
\ENDFOR
\FOR{each dummy record $rcd'$}
    \STATE $(Ercd, seed, \bm{n}, Grcd) \lt RcdEnc(rcd', 0)$ \label{code:mcdb-insert-enc-du}
    \STATE $INS_{IWS} \lt INS_{IWS} \cup (seed, \bm{n}, Grcd)$
    \STATE $INS_{SSS} \lt INS_{SSS} \cup Ercd$ \label{code:mcdb-insert-user-end}
\ENDFOR
\STATE Send $INS_{IWS}$ and $((\bm{E}_{f, g_f}, \tau_{f, g_f})^*)_{1 \leq f \leq F}$ to the IWS
\STATE Send $INS_{SSS}$ to the SSS

~\\

\STATE \underline{$SSS(INS_{SSS}$}):  \label{code:mcdb-insert-csp-be}
\STATE $IDs \lt \emptyset$
\FOR{each $Ercd \in INS_{SSS}$}
    \STATE $EDB(++id) \lt Ercd$  \label{code:mcdb-insert-csp-insert}
    \STATE $IDs \lt IDs \cup id$
\ENDFOR
\STATE Send $IDs$ to the IWS  \label{code:mcdb-insert-csp-end}

~\\

\STATE \underline{$IWS(INS_{IWS}, (\bm{E}_{f, g_f}, \tau_{f, g_f})^*)_{1 \leq f \leq F}, IDs)$}: \label{code:mcdb-insert-wss-be}
\FOR{each $(seed, \bm{n}, Grcd) \in INS_{IWS}$ and $id \in IDs$} \label{code:mcdb-insert-wss-seed}
    \STATE $NDB(id) \lt (seed, \bm{n})$
    \FOR{$f=1$ to $F$}
        \STATE $GDB (f, g_f) \lt (GDB(f, g_f).IL_{f, g_f} \cup id, (\bm{E}_{f, g_f}, \tau_{f, g_f})^*)$
        \label{code:mcdb-insert-wss-group}
    \ENDFOR
\ENDFOR  \label{code:mcdb-insert-wss-end}
%
\end{algorithmic}
%\end{multicols}
\end{algorithm}
%
%
\framework allows users to update the database after bootstrapping.
However, after updating, the occurrences of involved elements will change.
To effectively protect the search pattern, we should ensure the elements in the same group always have the same occurrence.
\framework achieves that by updating dummy records.
%The details for inserting a record is shown in Algorithm \ref{alg:mcdb-insert}.

\paragraph{Insert Query}
In \framework, the insert query is also performed with the cooperation of the user, IWS, and SSS.
The idea is that a number of dummy records will be generated and inserted with the real one to ensure all the elements in the same group always have the same occurrence.
The details are shown in Algorithm \ref{alg:mcdb-insert}.

Assume the real record to be inserted is $rcd=(e_1, \ldots, e_F)$.
The user encrypts it with \emph{RcdEnc}, and gets $(Ercd, seed, \bm{n}, Grcd)$ (Line \ref{code:mcdb-insert-user-enc}, Algorithm \ref{alg:mcdb-insert}).
For each $g_f \in Grcd$, the user gets $(\bm{E}_{f, g_f}, \tau_{f, g_f})^*$ of group $(f, g_f)$ and decrypts it.
Note that if $(f, g_f) \notin GDB$, the IWS returns $(\bm{E}_{f, g_f}, \tau_{f, g_f})^*$ of the closest group(s), instead of adding a new group.
That is, $e_f$ will belong to its closet group in this case.
The problem of adding new groups is that when the new groups contain less than $\lambda$ elements, adversaries could easily infer the search and access patterns within these groups.

The next step is to generate dummy records (Lines \ref{code:mcdb-insert-gendum-be}-\ref{code:mcdb-insert-gendum-end}).
The approach of generating dummy records depends on whether $e_f \in \bm{E}_{f, g_f}$, \ie whether $rcd$ introduces new element(s) that not belongs to $U$ or not.
If $e_f \in \bm{E}_{f, g_f}$, after inserting $rcd$, $O(e_f)$ will increase to $\tau_{f, g_f}+1$ automatically.
In this case, the occurrence of other elements in $\bm{E}_{f, g_f}$ should also be increased to $\tau_{f, g_f}+1$.
Otherwise, $O(e_f)$ will be unique in the database, and adversaries can tell if users are querying $e_f$ based on the size pattern.
To achieve that, $\gamma_f=|\bm{E}_{f, g_f}| -1$ dummy records are required for field $f$, and each of them contains an element in $\bm{E}_{f, g_f} \setminus e_f$.
%
If $e_f \notin \bm{E}_{f, g_f}$, $O(e_f)=0$ in $EDB$.
After inserting, we should ensure $O(e_f)=\tau_{f, g_f}$ since it belongs to the group $(f, g_f)$.
Thus, this case needs $\gamma_f=\tau_{f, g_f} -1$ dummy records for field $f$, and all of them are assigned with $e_f$ in field $f$.
%

Assume $W$ dummy records are required for inserting $rcd$, where $W=\max\{\gamma_f\}_{1 \leq f \leq F}$.
The user generates $W$ dummy records as mentioned above (`NULL' is used if necessary), and encrypts them with $RcdEnc$ (Lines \ref{code:mcdb-insert-encdum-be}-\ref{code:mcdb-insert-gendum-end}).
Meanwhile, the user adds each new element into the respective $\bm{E}_{f, g_f}$ if there are any, updates $\tau_{f, g_f}$, and re-encrypts $(\bm{E}_{f, g_f}, \tau_{f, g_f})$.
%The IWS can learn if $rcd$ includes new elements or not from the length of $(\bm{E}_{f, g_f}, \tau_{f, g_f})^*$. To avoid this leakage, the admin can pads $(\bm{E}_{f, g_f}, \tau_{f, g_f})^*$ to a fixed length when bootstrapping the database.
All the encrypted records are sent to the SSS and added into $EDB$ (Lines \ref{code:mcdb-insert-csp-be}-\ref{code:mcdb-insert-csp-end}).
All the $(seed, \bm{n})$ pairs and $(\bm{E}_{f, g_f}, \tau_{f, g_f})^*$ are sent to the IWS and inserted into $NDB$ and $GDB$ accordingly (Lines \ref{code:mcdb-insert-wss-be}-\ref{code:mcdb-insert-wss-end}).
%The SSS assigns an identifier $id$ to each $Ercd$ and stores it to $EDB(id)$.
%Recall that, to ensure the correctness of the search operation, the records in $EDB$ and their respective seeds and nonces in $NDB$ should have the same identifiers.
%Thus, the SSS sends the $id$ of each $Ercd$ to the IWS.
%After getting the $id$ for each $(seed, \bm{n}, Grcd)$ pair, the IWS stores $(seed, \bm{n})$ in $NDB(id)$, adds $id$ to each involved in $IL_{f, g_f}$, and increase each $\tau_{f, g_f}$ by one.
Finally, to protect the access pattern, the shuffling and re-randomising operations over the involved groups will be performed between the IWS and RSS.

\paragraph{Delete Query}
Processing delete queries is straightforward.
Instead of removing records from the database, the user sets them to dummy by replacing their $tag$s  with random strings.
In this way, the occurrences of involved elements are not changed.
Moreover, the correctness of the search result is guaranteed.
However, only updating the tags of matched records leaks the access pattern of delete queries to the RSS.
Particularly, the RSS could keep a view of the latest database and check which records' tags were modified when the searched records are sent back for shuffling.
%Moreover, the RSS knows these modified records are all dummy now.
To avoid such leakage, in \framework, the user modifies the tags of all the searched records for each delete query.
Specifically, the SSS returns the identifiers of matched records and the tags of all searched records to the user.
For matched records, the user changes their tags to random strings directly.
Whereas, for each unmatched records, the user first checks if it is real or dummy, and then generates a proper new tag as done in Algorithm~\ref{alg:mcdb-enc}.
Likewise, the \emph{PreShuffle} and \emph{Shuffle} algorithms are performed between the IWS and RSS after updating all the tags.

However, if the system never removes records, the database will increase rapidly.
To avoid this, the admin periodically removes the records consisting of $F$ `NULL' from the database.
Specifically, the admin periodically checks if each element in each group is contained in one dummy record.
If yes, for each element, the admin updates one dummy record containing it to `NULL'.
As a consequence, the occurrence of all the elements in the same group will decrease, but still is the same.
When the dummy record only consists of `NULL', the admin removes it from the database.

\paragraph{Update query}
In \framework, update queries can be performed by deleting the records with old elements and inserting new records with new elements.


==> PMcDb_arXiv/sections/intro.tex <==
\section{Introduction}
\label{sec:introduction}
Cloud computing is a successful paradigm offering companies and individuals virtually unlimited
data storage and computational power at very attractive costs.
However, uploading sensitive data, such as medical, social, and financial information, to public cloud environments is still a challenging issue due to security concerns.
In particular, once such data sets and related operations are uploaded to cloud environments, the tenants must therefore trust the Cloud Service Providers (CSPs).
Yet, due to possible cloud infrastructure bugs~\cite{GunawiHLPDAELLM14}, misconfigurations~\cite{dropboxleaks} and external attacks~\cite{verizonreport}, the data could be disclosed or corrupted.
Searchable Encryption (SE) is an effective approach that allows organisations to outsource their databases and search operations to untrusted CSPs, without compromising the confidentiality of records and queries.
%The basic idea is to encrypt the data using Searchable Encryption (SE) schemes before sending to the CSPs.

Since the seminal SE paper by Song \etal \cite{Song:2000:Practical}, a long line of work has investigated SE schemes with flexible functionality and better performance \cite{Asghar:2013:CCSW,Curtmola:2006:Searchable,Popa:2011:Cryptdb,Sarfraz:2015:DBMask}.
These schemes are proved to be secure in certain models under various cryptographic assumptions.
Unfortunately, a series of more recent work \cite{Islam:2012:Access,Naveed:2015:Inference,Cash:2015:leakage,Zhang:2016:All,Kellaris:ccs16:Generic,Abdelraheem:eprint17:record}
illustrates that they are still vulnerable to inference attacks, where malicious CSPs could recover the content of queries and records by (i) observing the data directly from the encrypted database and (ii) learning about the results and queries when users access the database.
% also the information about the results and queries learned during access by users to the database.

%Roughly speaking,
From the encrypted database, the CSP might learn the frequency information of the data.
From the search operation, the CSP is able to know the \emph{access pattern}, \ie the records returned to users in response to given queries.
The CSP can also infer if two or more queries are equivalent, referred to as the \emph{search pattern}, by comparing the encrypted queries or matched data.
Last but not least, the CSP can simply log the number of matched records or files returned by each query, referred to as the \emph{size pattern}.

When an SE scheme supports insert and delete operations, it is referred to as a \emph{dynamic} SE scheme.
Dynamic SE schemes might leak extra information if they do not support \emph{forward privacy} and \emph{backward privacy} properties.
Lacking forward privacy means that the CSP can learn if newly inserted data or updated data matches previously executed queries.
Missing backward privacy means that the CSP learns if deleted data matches new queries.
Supporting forward and backward privacy is fundamental to limit the power of the CSP to collect information on how the data evolves over time.
However, only a few schemes \cite{BostMO17,ZuoSLSP18,ChamaniPPJ18,AmjadKM19} ensure both properties simultaneously.

Initiated by Islam \etal (IKK)\cite{Islam:2012:Access}, more recent works \cite{Cash:2015:leakage,Naveed:2015:Inference,Zhang:2016:All,Kellaris:ccs16:Generic} have shown that such leakage can be exploited to learn sensitive information and break the scheme.
Naveed \etal \cite{Naveed:2015:Inference} recover more than $60\%$ of the data in CryptDB \cite{Popa:2011:Cryptdb} using frequency analysis only.
Zhang \etal \cite{Zhang:2016:All} further investigate the consequences of leakage by injecting chosen files into the encrypted storage.
Based on the access pattern, they could recover a very high fraction of searched keywords by injecting a small number of known files.
Cash \etal \cite{Cash:2015:leakage} give a comprehensive analysis of the leakage in SE solutions for file collection and introduced the \emph{count attack}, where an adversary could recover queries by counting the number of matched records even if the encrypted records are semantically secure.

%Another issue with SE schemes is the key management mechanism to flexibly support multiple user access.
%Some schemes, like \cite{Curtmola:2006:Searchable}, encrypt the data and queries with the key shared among all the users.
%Consequently, all the queries and search results issued by one user could be decrypted by all authorised users.
%Even worse, when one user is revoked, the single key has to be changed and the data has to be re-encrypted with the new key.
%In other schemes, such as \cite{Cao:2014:Privacy} and \cite{Wang:2015:Inverted}, the keys are only known to the data owner.
%The users have to send the query and search results to the data owner to get the search tokens and cleartext results, which means that the data owner represents a bottleneck in the system.

In this article, we investigate the leakage and attacks against relational databases\footnote{In the rest of this article, we use the term \emph{database} to refer to a relational database.} and present a \underline{P}rivacy-preserving \underline{M}ulti-\underline{c}loud based dynamic SSE scheme for \underline{D}ata\underline{b}ases (\framework).
\framework can effectively resist attacks based on the search, size or/and access patterns.
Our key technique is to use three non-colluding cloud servers: one server stores the data and performs the search operation, and the other two manage re-randomisation and shuffling of the database for protecting the access pattern.
%\todo[inline]{Mention here what we achieve with `re-randomisation and shuffling of the database'.}
A user with access to all servers can perform an encrypted search without leaking the search, access, or size pattern.
When updating the database, \framework also ensures both forward and backward privacy.
We give full proof of security against honest-but-curious adversaries and show how \framework can hide these patterns effectively.

%Furthermore, we handle the situation where many users have access to the same database. Each user is able to protect her queries and search results against all the other entities. Last but not least, \framework is more efficient for user revocation than most of the existing SE schemes: instead of changing the key and re-encrypting the data, we only need to inform all the CSPs to stop any service for the revoked user. Although the revoked users still own the key, they are unable to issue queries or recover the data even if they collude with one of the CSPs.

The contributions of this article can be summarised as follows:
\begin{itemize}

    \item %{\color{blue}
    We provide leakage definition specific to searchable encrypted databases, and then review how existing attacks leverage the leakage to recover queries and records. %}

   \item We propose a privacy-preserving SSE database \framework, which protects the search, access, and size patterns, and achieves both forward and backward privacy, thus ensuring protection from leakage-based attacks.

  %\item \framework supports flexible multi-user access in a way that the issued queries and search results of one user are protected from other entities. Moreover, revoking users do not require key regeneration and data re-encryption even when one of the CSPs colludes with revoked users.

  \item %{\color{blue}
  We give full proof of security against honest-but-curious adversaries and show how \framework can effectively hide these patterns and resist leakage-based attacks.%}

    \item %{\color{blue}
    Finally, we implement a prototype of \framework and show its practical efficiency by evaluating its performance on TPC-H dataset. %}
\end{itemize}

The rest of this article is organised as follows.
In Section~\ref{sec:notation}, we define notations.
We present the leakage levels in SE schemes and review leakage-based attacks in Section~\ref{sec:leakage}.
In Section~\ref{sec:overview}, we provide an overview of \framework.
Solution details can be found in Section~\ref{sec:MCDB-details}.
In Section~\ref{sec:security}, we analyse the security of \framework.
Section~\ref{sec:MCDB-perf} reports the performance of \framework.
Finally, we conclude this article in Section~\ref{sec:conclusion}.


==> PMcDb_arXiv/sections/leakage.tex <==
\section{Leakage and Attacks}
\label{sec:leakage}
\subsection{Leakage Definition}
%\todo[inline]{This section needs to be updated based on updated definitions.}
In \cite{Cash:2015:leakage}, Cash \etal define four different levels of leakage profiles for encrypted file collections according to the method of encrypting files and the data structure supporting encrypted search.
Yet, we cannot apply these definitions to databases directly, since the structure of a file is different from that of a record in the database.
In particular, a file is a collection of related words arranged in a semantic order and tagged with a set of keywords for searching; whereas, a record consists of a set of keywords with predefined attributes.
Moreover, a keyword may occur more than once in a file, and different keywords may have different occurrences; whereas, a keyword of an attribute generally occurs only once in a record.
Inspired by the leakage levels defined in \cite{Cash:2015:leakage}, in this section, we provide our own layer-based leakage definition for encrypted databases.
Specifically, we use the terminology \emph{leakage} to refer to the information the CSP can learn about the data directly from the encrypted database and the information about the results and queries when users are accessing the database.

The simplest type of SE scheme for databases is encrypting both the records and queries with Property-Preserving Encryption (PPE), such as the DETerministic (DET).
In DET-based schemes, the same data has the same ciphertext once encrypted.
In this type of SE schemes, the CSP can check whether each record matches the query efficiently by just comparing the corresponding ciphertext; however, these solutions result in information leakage.
Specifically, in DET-based schemes, such as CryptDB \cite{Popa:2011:Cryptdb} (where the records are protected only with the PPE layer), DBMask \cite{Sarfraz:2015:DBMask}, and Cipherbase \cite{Arasu:CIDR13:Cipherbase}, before executing any query, the CSP can learn the data distribution, \ie the number of distinct elements and the occurrence of each element, directly from the ciphertext of the database.
Formally, we say the data distribution of $DB$ is leaked if $e^*$ and $e$ have the same occurrence, \ie $O(e)=O(e^*)$, for each $e \in U$.
%, where $e^*$ is the ciphertext of $e$ in $EDB$.
%In this article, we focus on the equality queries.
We define this leakage profile set as $\mathcal{L}_3$:
%
\begin{itemize}
  \item $\mathcal{L}_3=\{O(e)\}_{e \in U}$.
\end{itemize}
%Note that L3 leakage does not require any queries at all, the CSP learns this directly from EDB

The second type of SE for databases encrypts the data with semantically secure primitives, but still encrypts the queries with DET encryption.
By doing so, the data distribution is protected, and the CSP can still search the encrypted database efficiently by repeating the randomisation over the DET query and then comparing it with the randomised data, as done in \cite{Hahn:2014:Searchable}, Arx \cite{Poddar:arx:eprint16}, and most of the Public-key Encryption with Keyword Search (PEKS) systems, such as \cite{BonehCOP04} and BlindSeer \cite{Fisch:SP15:BlindSeer}.
%\todo[inline]{Should we also include PEKS here?}
However, after executing a query, the CSP could still learn the access and size patterns.
Moreover, due to the DET encryption for queries, the search pattern is also leaked.
Given a sequence of $q$ queries $\textbf{Q}=(Q_1, \ldots, Q_q)$, we define the leakage profile as:
\begin{itemize}
  \item $\mathcal{L}_2=\{|DB(Q_i)|, \{EDB(Q_i)\cap EDB(Q_j), Q_i\stackrel{?}{=}Q_j\}_{Q_j \in \bm{Q}}\}_{Q_i \in \textbf{Q}}$
\end{itemize}
%
Note that after executing queries, PPE-based databases also leak the profiles included in $\mathcal{L}_2$.

A more secure SE solution leverages Oblivious RAM (ORAM)  \cite{Goldreich:1996:SPS,Stefanov:2013:PathORAM} or combines Homomorphic Encryption (HE) \cite{Paillier:1999:Public,Gentry:2009:FHE} with oblivious data retrieval to hide the search and access patterns.
For instance, the HE-based $PPQED_a$ proposed by Samanthula \etal \cite{Samanthula:2014:Privacy} and the ORAM-based SisoSPIR given by Ishai \etal \cite{Ishai:2016:Private} hide both the search and access patterns.
%Specifically, to hide the data distribution and the search pattern, both $PPQED_a$ and SisoSPIR randomise the encrypted records and queries.
%To conceal the access pattern from the CSP, in $PPQED_a$, the match result between records and queries is encrypted and can only be learned by the user.
%Furthermore, the matched records are loaded through oblivious transfer protocols.
%Thus, the CSP never learns which records match the query.
%In SisoSPIR, whether each record matches the query is checked by the user, and the access pattern is protected by using ORAM.
Unfortunately, in both schemes, the CSP can still learn how many records are returned to the user after executing a query, \ie \emph{the communication volume}.
According to \cite{Kellaris:ccs16:Generic}, the HE-based and ORAM-based SE schemes have fixed communication overhead between the CSP and users.
Specifically, the length of the message sent from the CSP to the user as the result of query execution is proportional to the number of records matching the query.
Based on this observation, the CSP can still infer the size pattern.
Thus, the HE-based and ORAM-based SE schemes are vulnerable to size pattern-based attacks, \eg count attack \cite{Cash:2015:leakage}.
The profile leaked in HE-based and ORAM-based SE schemes can be summarised below:
\begin{itemize}
  \item $\mathcal{L}_1=\{|DB(Q_i)|\}_{Q_i \in \bm{Q}}$.
\end{itemize}

%In addition, to maintain search functionality, it is hard to avoid leaking the basic knowledge of the database and queries. For instance, to allow searching over different fields, existing schemes \cite{Popa:2011:Cryptdb} and \cite{Asghar:2013:CCSW} encrypt each data element individually. Therefore, they leak the number of records and fields in the database and the fields searched by each query. Moreover, in order to let the CSP know what kind of operation to execute, almost all the existing SE schemes keep the query type (\eg select, insert, delete or update) and operator (\eg $=$, $<$ or $>$) in plaintext. Herein, we define these types of basic leakage as $\mathcal{L}_0$:
%\begin{itemize}
%  \item $\mathcal{L}_0=\{|EDB|, F, \{Q_i.f, Q_i.type, Q_i.op\}_{Q_i \in \textbf{Q}}\}$.
%\end{itemize}


==> PMcDb_arXiv/sections/notation.tex <==
\section{Notations and Definitions}
\label{sec:notation}
%
\begin{table}
\centering
\caption{Notation and description}
\scriptsize
\label{tbl:notation}
\begin{tabular}{|l|l|} \hline
\textbf{Notation}   & \textbf{Description}  \\ \hline
$e$        & Data element \\ \hline
$|e|$      &The length of data element \\ \hline
$F$        & Number of attributes or fields  \\ \hline
$rcd_{id}=(e_{id, 1}, \ldots, e_{id, F})$ & The $id$-th record  \\ \hline
$N$        & Number of records in the database  \\ \hline
$DB=\{rcd_1, \ldots, rcd_N\}$             & Database  \\ \hline
$DB(e)=\{rcd_{id} | e \in rcd_{id}\}$  & Records containing $e$ in $DB$  \\ \hline
$O(e)=|DB(e)|$                         & Occurrence of $e$ in $DB$  \\ \hline
$U_f=\cup \{e_{id, f}\}$  & The set of distinct elements in field $f$  \\ \hline
$U=\{U_{1}, ..., U_F\}$   & All the distinct elements in $DB$  \\ \hline
$e^*$      & Encrypted element  \\ \hline
$Ercd$     & Encrypted record   \\ \hline
$EDB$      & Encrypted database  \\ \hline
$Q=(type, f, e)$             & Query  \\ \hline
$Q.type$   & `select' or `delete' \\ \hline
$Q.f$      & Identifier of interested field  \\ \hline
$Q.e$      & Interested keyword   \\ \hline
$EQ$        & Encrypted query  \\ \hline
$EDB(EQ)$ or $EDB(Q)$   & Search result of $Q$  \\ \hline
$(f, g)$   & Group $g$ in field $f$  \\ \hline
$\bm{E}_{f,g}$ & Elements included in group $(f,g)$ \\ \hline
$\tau_{f,g}=\max \{O(e)\}_{e \in \bm{E}_{f, g}}$ & Threshold of group $(f, g)$ \\ \hline
$(\bm{E}_{f,g}, \tau_{f,g})^*$ & Ciphertext of $(\bm{E}_{f,g}, \tau_{f,g})$ \\ \hline
\end{tabular}

We say $EQ(Ercd)=1$ when $Ercd$ matches $EQ$.
Thus, the search result $EDB(EQ) = \{Ercd_{id} | EQ(Ercd_{id})=1\}$.
\end{table}
%
%
In this section, we give formal definitions for the search, access, and size patterns, as well as for forward and backward privacy.
Before that, in Table~\ref{tbl:notation}, we define the notations used throughout this article.

%
\begin{mydef}[\textbf{Search Pattern}]
%\todo[inline]{What do you mean by `a polynomial size'?}
Given a sequence of $q$ queries $\bm{Q}=(Q_1, \ldots, Q_q)$, the search pattern of $\bm{Q}$ represents the correlation between any two queries $Q_i$ and $Q_j$, \ie $\{Q_i\stackrel{?}{=}Q_j\}_{Q_i, Q_j \in \bm{Q}}$\footnote{$Q_i=Q_j$ only when $Q_i.type=Q_j.type$, $Q_i.f=Q_j.f$, and $Q_i.e=Q_j.e$}, where $1 \leq i, j \leq q$.
\end{mydef}
%\todo[inline]{To be more precise, also specify constraints over i and j, \ie i,j are greater than or equal to 1 and less than or equal to q.}
%

In previous works, access pattern is generally defined as the records matching each query \cite{Curtmola:2006:Searchable}, \ie the search result.
In fact, in leakage-based attacks, such as \cite{Zhang:2016:All,Islam:2012:Access,Cash:2015:leakage}, the attackers leverage the intersection between search results (explained in Section \ref{sec:attack}) to recover queries, rather than each single search result.
Therefore, in this work, we define the intersection between search results as access pattern.

\begin{mydef}[\textbf{Access Pattern}]
The access pattern of $\bm{Q}$ represents the intersection between any two search results, \ie $\{EDB(Q_i) \cap EDB(Q_j)\}_{Q_i, Q_j \in \bm{Q}}$.
\end{mydef}
%
\begin{mydef}[\textbf{Size Pattern}]
The size pattern of $\bm{Q}$ represents the number of records matching each query, \ie $\{|DB(Q_i)|\}_{Q_i\in \bm{Q}}$.
\end{mydef}
%
\begin{mydef}[\textbf{Forward Privacy}]
Let $Ercd^t$ be an encrypted record inserted or updated at time $t$, a dynamic SE scheme achieves forward privacy, if $EQ(Ercd^t)\stackrel{?}{=}0$ is always true for any query $EQ$ issued at time $t^*$, where $t^* < t$.
%\todo[inline]{Note that I have made this definition a bit more formal.Double check.}
\end{mydef}
%
\begin{mydef}[\textbf{Backward Privacy}]
Let $Ercd^t$ be an encrypted record deleted at time $t$, a dynamic SE scheme achieves backward privacy, if $EQ(Ercd^t)\stackrel{?}{=}0$ is always true for any query $EQ$ issued at time $t'$, where $t < t'$.
%\todo[inline]{Note that I have made this definition a bit more formal. Double check.}
\end{mydef}
%


==> PMcDb_arXiv/sections/overview.tex <==
\section{Overview of \framework}
\label{sec:overview}
In this work, we propose \framework, a multi-cloud based dynamic SSE scheme for databases that can resist the aforementioned leakage-based attacks. % by minimising the leakage to $\mathcal{L}'_0$, a new level that approximates to $\mathcal{L}_0$.
Specifically, our scheme not only hides the frequency information of the database, but also protects the size, search, and access patterns.
Moreover, it ensures both forward and backward privacy when involving insert and delete queries.
Comparing with the existing SE solutions, \framework has the smallest leakage.
%As far as we know, \framework is the first SE scheme that can resist leakage-based attacks, including the active file/record-injection attack.}
In this section, we define the system and threat model, and illustrate the techniques used in \framework at high-level.

\subsection{System Model}
\label{subsec:sm}
\begin{figure}
  \centering
  \includegraphics[width=.5\textwidth]{figs/arch.pdf}\\
  \caption{An overview of \framework:
  Users can upload records and issue queries.
  The SSS, IWS, and RSS represent independent CSPs.
  The SSS stores encrypted records and executes queries.
  The IWS stores index and auxiliary information, and provides witnesses to the SSS for performing encrypted search.
  After executing each query, the SSS sends searched records to the RSS for shuffling and re-randomising to protect patterns privacy.}
  \label{Fig:arch}
\end{figure}
%
In the following, we define our system model to describe the entities involved in \framework, as shown in Fig.~\ref{Fig:arch}:

 \begin{itemize}

   \item \textbf{Admin}: An admin is responsible for the setup and maintenance of databases, user management as well as specification and deployment of access control policies.

   \item \textbf{User}: A user can issue insert, select, delete, and update queries to read and write the database according to the deployed access control policies.
       \framework allows multiple users to read and write the database.
       %Users can also decrypt search results they get in response to their queries.

   \item \textbf{Storage and Search Service (SSS)}:
   It provides encrypted data storage, executes encrypted queries, and returns matching records in an encrypted manner.

   \item \textbf{Index and Witness Service (IWS)}:
    It stores the index and auxiliary information, and provides witnesses to the SSS for retrieving data.
    The IWS has no access to the encrypted data.

   \item \textbf{Re-randomise and Shuffle Service (RSS)}:
    After executing each query, it re-randomises and shuffles searched records to achieve the privacy of access pattern.
    The RSS does not store any data.

 \end{itemize}
    %\item \textbf{Cloud Service Providers (CSPs)}:
    Each of the SSS, IWS, and RSS is deployed on the infrastructure managed by CSPs that are in conflict of interest. 
    According to the latest report given by RightScale \cite{RightScale:2016:report}, organisations are using more than three public CSPs on average, which means the schemes based on multi-cloud are feasible for most organisations. 
    The CSPs have to ensure that there is a two-way communication between any two of them, but our model assumes there is no collusion between the CSPs.

\subsection{Threat Model}
\label{subsec:tm}
We assume the admin is fully trusted.
All the users are only assumed to securely store their keys and the data.
%, however, malicious and revoked users may try to learn what other users are searching for and the result set, or they can collude with the SSS or IWS (or the CSPs hosting them) to get access to the data they otherwise are not authorised to access.

The CSPs hosting the SSS, IWS, and RSS are modelled as honest-but-curious.
More specifically, they honestly perform the operations requested by users according to the designated protocol specification.
However, as mentioned in the above leakage-based attacks, they are curious to gain knowledge of records and queries by 1) analysing the outsourced data, 2) analysing the information leaked when executing queries, 3) and injecting malicious records.
As far as we know, \framework is the first SE scheme that considers active CSPs that could inject malicious records. 
Moreover, as assumed in \cite{Samanthula:2014:Privacy,Hoang:2016:practical,Stefanov:CCS2013:Multi-cloud}, we also assume the CSPs do not collude.
In other words, we assume an attacker could only compromise one CSP. 
In practice, any three cloud providers in conflict of interest, such as Amazon S3, Google Drive, and Microsoft Azure, could be considered since they may be less likely to collude in an attempt to gain information from their customers. 

We assume there are mechanisms in place for ensuring data integrity and availability of the system.
%Last but not least, access policy specification is out of the scope of this paper. %, but the approach introduced in \cite{Asghar:2013:CCSW, Asghar:2013:phdthesis} can be utilised in \framework.
%In the rest of our discussion, we will refer to the each CSPs as IWS or SSS depending on what service they are hosting.

\subsection{Approach Overview}
\label{subsec:appo}
\framework aims at hiding the search, access, and size patterns.
\framework also achieves both backward and forward privacy.
%In \framework, it is efficient to revoke users because no key re-generation and data re-encryption operations are needed.
We now give an overview of our approach.

To protect the search pattern, \framework XORs the query with a nonce, making identical queries look different once encrypted (\ie the encrypted query is semantically secure).
However, the CSP may still infer the search pattern by looking at the access pattern.
Specifically, the CSP can infer that two queries are equivalent if the same records are returned.
To address this issue, after executing each query, we shuffle the locations of the searched records.
Moreover, we re-randomise their ciphertexts, making them untraceable.
In this way, even if a query equivalent to the previous one is executed, the CSP will see a new set of records being searched and returned, and cannot easily infer the search and access pattern.
%This also implies that the search pattern remains protected.

Another form of leakage is the size pattern, where the CSP can learn the number of records returned after performing a query, even after shuffling and re-randomisation.
Moreover, the CSP can guess the search pattern from the size pattern.
Specifically, the queries matching different numbers of records must be different, and the queries matching the same number of records could be equivalent.
To protect the size pattern, we introduce a number of dummy records that look exactly like the real ones and could match queries.
Consequently, the search result for each query will contain a number of dummy records making it difficult for the CSP to identify the actual number of real records returned by a query.

To break the link between size and search pattern, our strategy is to ensure all queries always match the same number of records, and the concrete method is to pad all the data elements in each field into the same occurrence with dummy records.
By doing so, the size pattern is also protected from the communication volume since there is no fixed relationship between them.
However, a large number of dummy records might be required for the padding.
To reduce required dummy records and ensure \framework's performance, we virtually divide the distinct data elements into groups and only pad the elements in the same group into the same occurrence.
By doing so, the queries searching values in the same group will always match the same number of records.
Then, the CSP cannot infer their search pattern.
Here we clarify that the search pattern is not fully protected in \framework.
Specifically, the CSP can still tell the queries are different if their search results are in different groups.

\framework also achieves forward and backward privacy.
Our strategy is to blind records also with nonces and re-randomise them using fresh nonces after executing each query.
Only queries that include the current nonce could match records.
In this way, even if a malicious CSP tries to use previously executed queries with old nonces, they will not be able to match the records in the dataset, ensuring forward privacy.
Similarly, deleted records (with old nonces) will not match newly issued queries because they use different nonces.
%The use of nonces also limits the records that a revoked user could be able to access even if she is able to access the encrypted data.

The details and algorithms of our scheme will be discussed in the following section.


==> PMcDb_arXiv/sections/performance.tex <==
\section{Performance Analysis}
\label{sec:MCDB-perf}
We implemented \framework in C using MIRACL 7.0 library for cryptographic primitives.
%Specifically, the encryption $Enc$, the PRG $\Gamma$ and hash function $H$ are implemented with AES-128, keyed hash SHA-512, and SHA-128 respectively.
The performance of all the entities was evaluated on a desktop machine with Intel i5-4590 3.3 GHz 4-core processor and 8GB of RAM.
We evaluated the performance using TPC-H benchmark \cite{TPC:2017:h}, and tested equality queries with one singe predicates over `O\_CUSTKEY' field in `ORDERS' table.
In the following, all the results are averaged over $100$ trials.

\subsection{Group Generation}
\begin{table}[h]
%\small
\scriptsize
  \centering
    \caption{The storage overhead with different numbers of groups}
  \begin{tabular}{|l|l|l|l|l|}
     \hline
     % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
     \#Groups  &\#Dummy records &\#Elements in a group & \#Records in a group  \\ \hline
     1         & 2599836 & 99996 & =4099836  \\
     10        & 2389842 & 10000 & $\approx$38000 \\
     100       & 1978864 & 1000  & $\approx$35000  \\
     1000      & 1567983 & 100   & $\approx$3000  \\
     10000     & 1034007 & 10    & $\approx$240 \\
     \hline
   \end{tabular}
  \label{Tbl:oblidb-storage-perf}
\end{table}
%
In `ORDERS' table, all the `O\_CUSTKEY' elements are integers.
For simplicity, we divided the records into groups by computing $e~ mod~ b$ for each element $e$ in `O\_CUSTKEY' field.
Specifically, we divide the records into 1, 10, 100, 1000, and 10000 groups by setting $b=$1, 10, 100, 1000,  and 10000, respectively.

%As mentioned in Section \ref{subsec:boot}, both the number of required dummy records and the security level of \framework vary with the way of grouping.
Table \ref{Tbl:oblidb-storage-perf} shows the number of required records and the number of elements included in a group when dividing the database into 1, 10, 100, 1000, and 10000 groups.
In particular, when all the records are in one group, $2599836$ dummy records are required in total, $\lambda=99996$, and the CSP has to search $4099836$ records for each query.
% and the scheme ensures the highest level of security, where the two queries matching the same number of records are identical with $10^{-5}$ probability. However
When we divide the records into more groups, fewer dummy records are required, fewer records will be searched by the CSP, but fewer elements will be contained in each group.
When there are $10000$ groups, only $1034007$ dummy records are required totally, $\lambda=10$, and the CSP just needs to search around $240$ records for each query.
%However, $\lambda=10$ in this case, \ie the queries matching the same number of records are identical with $0.1$ probability.


\subsection{Query Latency}
%
\begin{figure}[htp]
\centering
\includegraphics[width=0.32\textwidth]{figs/entity.pdf}\\
\caption{The overhead on different entities with different group numbers}
\label{Fig:mcdb-entity}
\end{figure}
%
An important aspect of an outsourced service is that most of the intensive computations should be off-loaded to the CSPs.
To quantify the workload on each of the entities, we measured the latency on the user, IWS, SSS, and RSS for processing the query with different numbers of groups.
The results are shown in Fig.~\ref{Fig:mcdb-entity}.
We can notice that the computation times taken on the IWS, SSS, and RSS are much higher than that on the user side when there are less than 10000 groups.
In the following, we will discuss the performance on CSPs and the user in details.


\subsubsection{Overhead on CSPs}
%
\begin{figure}[htp]
\centering
\includegraphics[width=0.32\textwidth]{figs/CSPs.pdf}\\
\caption{The overhead on CSPs with different group numbers}
\label{Fig:mcdb-csps}
\end{figure}
%
Fig. \ref{Fig:mcdb-csps} shows the performance of the operations running in the CSPs when increasing the number of groups.
Specifically, in \framework, the IWS runs \emph{NonceBlind} and \emph{PreShuffle}, the SSS runs \emph{Search}, and the RSS runs \emph{Shuffle} algorithms.
We can notice that the running times of all the four operations reduce when increasing the number of groups.
The reason is that \framework only searches and shuffles a group of records for each query.
The more groups, the fewer records in each group for searching and shuffling.
Thanks to the efficient XOR operation, even when $g=1$, \ie searching the whole database (contains 4099836 records in total), \emph{NonceBlind}, \emph{Search}, and \emph{Shuffle} can be finished in around $2$ seconds.
\emph{PreShuffle} is the most expensive operation in \framework, which takes about $11$ seconds when $g=1$.
Fortunately, in \emph{PreShuffle}, the generation of new nonces (\ie Lines \ref{code:mcdb-seed'}-\ref{code:mcdb-gn'} in Algorithm \ref{alg:mcdb-shuffle}) is not affected by the search operation, thus they can be pre-generated.
By doing so, \emph{PreShuffle} can be finished in around $2.4$ seconds when $g=1$.
%the throughput of \framework can be improved significantly.


\subsubsection{Overhead on Users}
%
\begin{figure}[htp]
\centering
\includegraphics[width=0.32\textwidth]{figs/user_group.pdf}\\
\caption{The overhead on the user with different group numbers}
\label{Fig:mcdb-user}
\end{figure}
%
In \framework, the user only encrypts queries and decrypts results.
In Fig. \ref{Fig:mcdb-user}, we show the effect on the two operations when we change the number of groups.
The time for encrypting the query does not change with the number of groups.
However, the time taken by the result decryption decreases slowly when increasing the number of groups.
For recovering the required records, in \framework, the user first filters out the dummy records and then decrypts the real records.
Therefore, the result decryption time is affected by the number of returned real records as well as the dummy ones.
In this experiment, the tested query always matches 32 real records.
However, when changing the number of groups, the number of returned dummy records will be changed.
Recall that, the required dummy records for a group is $\sum_{e \in \bm{E}_{f, g}}(\tau_{f, g}-O(e))$, and the threshold $\tau_{f, g}=\max\{O(e)\}_{e \in \bm{E}_{f, g}}$.
%The group threshold $\tau_{i,f}$ is determined by the highest occurrence in the group.
When the records are divided into more groups, fewer elements will be included in each group.
As a result, the occurrence of the searched element tends to be closer to $\tau_{f, g}$, and then fewer dummy records are required for its padding.
Thus, the result decryption time decreases with the increase of the group number.
In the tested dataset, the elements have very close occurrences, which ranges from $1$ to $41$.
The number of matched dummy records are $9$, $9$, $2$, $1$, and $0$ when there are $1$, $10$, $100$, $1000$, and $10000$ groups, respectively.
For the dataset with a bigger element occurrence gap, the result decryption time will change more obviously when changing the number of groups.


\subsubsection{End-to-end Latency}
Fig. \ref{Fig:mcdb-user} also shows the end-to-end latency on the user side when issuing a query.
In this test, we did not simulate the network latency, so the end-to-end latency shown here consists of the query encryption time, the nonce blinding time, the searching time and the result decrypting time.
The end-to-end latency is dominated by the nonce blinding and searching times, thus it decreases when increasing the number of groups.
Specifically, the end-to-end query decreases from $2.16$ to $0.0006$ seconds when the number of groups increases from $1$ to $10000$.

In this test, we used one trick to improve the performance.
As described in Algorithm \ref{alg:macdb-search}, the SSS is idle before getting $(IL, EN)$.
Indeed, the IWS can send $IL$ to the SSS first, and then the SSS can pre-compute $temp_{id}=H'(EDB(id, EQ.f) \oplus EQ.e^*)$ while the IWS generating $EN$.
After getting $EN$, the SSS just needs to check if $temp_{id}=EN(id).w$.
By computing $(w, t)$ and $temp$ simultaneously, the user can get the search result more efficiently.
In this test, the SSS computed $t$ simultaneously when the IWS generating $EN$.
Note that the shuffle operation does not affect the end-to-end latency on the user side since it is performed after returning search results to users.

\subsection{Insert and Delete Queries}
\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=.32\textwidth]{figs/insdelsel.pdf}\\
  \caption{The execution times of the insert, delete and select queries with different numbers of groups}
  \label{Fig:mcdb-insert}
\end{figure}
%
\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=.3\textwidth]{figs/insdelsel_result.pdf}\\
  \caption{The execution times of the insert, delete, and select queries with different result sizes}
  \label{Fig:mcdb-insert-result}
\end{figure}
%
Since \framework is a dynamic SE scheme, we also tested its performance for insert and delete queries.

In Fig. \ref{Fig:mcdb-insert}, we show the execution times of insert and delete when changing the number of groups\footnote{The times taken by the $PreShuffle$ and $Shuffle$ algorithms are not included.}.
Moreover, we take the end-to-end latency of select queries as the baseline.
Fig. \ref{Fig:mcdb-insert} shows both insert and delete queries execute faster when there are more groups.
For insert queries, as mentioned in Section \ref{subsec:update}, $W=\max\{\gamma_{f}\}_{1 \leq f \leq F}$ dummy records should be inserted when inserting a real record.
Thus, the performance of insert queries is affected by the number of elements in involved groups.
When the database is divided into more groups, the fewer elements will be included in each group.
In this experiment, when there are 1, 10, 100, 1000, and 10000 groups, the user has to generate and encrypt 99996, 10000, 1000, 100, and 10 dummy records, respectively.
Specifically, when there is only one group, \framework takes only around $1.5$ seconds to encrypt and insert $99997$ records, which is slightly better than select queries.

For delete queries, \framework first performs the search operation to get the matched records, and then turn them to dummy by changing the tags.
Moreover, to hide the access pattern from the RSS, the user also needs to change the tags of all the other searched records.
The more groups, the fewer records should be searched, and the fewer tags should be changed.
Therefore, the performance of delete queries also gets better when there are more groups.
However, comparing with select queries, delete queries takes much longer time to change the tags.
Specifically, it takes around $20$ seconds to execute a delete query when there is only one group.

We also tested how the result size affects the performance of select and delete queries.
For this test, we divided the database into 10 groups, and the searched group contains $360000$ records.
Moreover, we manually changed the data distribution in the group to be searched to ensure that we can execute queries matching $36$, $360$, $3600$, $36000$, $360000$ records.
From Fig. \ref{Fig:mcdb-insert-result}, we can see that the performance of delete queries is better when the result size is bigger.
The reason is that tags of matched records are processed in a much efficient way than unmatched records.
Specifically, as mentioned in Section \ref{subsec:update}, the user directly changes the tags of matched records to random strings.
However, for each unmatched record, the user first has to detect if it is dummy or not, and then update their tags accordingly.
When all the searched records match the delete query, it takes only $0.6$ seconds to turn them to dummy.
Nonetheless, select queries take longer time when more records matching the query, since there are more records should be processed on the user side.

%Note that, in Fig.~\ref{Fig:mcdb-insert}, we do not include the time for running the $Shuffle$ algorithm. %However, it is necessary to hide the access pattern.

\iffalse
\subsection{Comparison with Other Schemes}
To better investigate the performance of our approach, here we roughly compare the search time of \framework with $PPQED_a$ and SisoSPIR.
Although we did not access their implementation, our experiments were conducted on Linux machines with approximate power\footnote{$PPQED_a$ was tested on a Linux machine with an
Intel Xeon 6-Core CPU 3.07 GHz processor and 12 GB RAM and SisoSPIR was tested on a machine with an Intel i7-2600K 3.4GHz 4-core CPU 8GB RAM.}.
Searching over 1 million records takes more than 10 seconds in SisoSPIR.
In $PPQED_a$, it takes 1 second to check if a predicate matches with a record when the data size is $10$ bits.
However, \framework only takes less than 2 seconds when searching over 4.1 million records, which is much more efficient than the other two schemes.
\fi


==> PMcDb_arXiv/sections/proof.tex <==
\section{Security Analysis}
\label{sec:security}
In this section, we first analyse the leakage in \framework.
Second, we prove the patterns and forward and backward privacy are protected against the CSPs.

\subsection{Leakage of \framework}
Roughly speaking, given an initial database $DB$ and a sequence of queries $\bm{Q}$, the information leaked to each CSP in \framework can be defined as:
\begin{align*}
\mathcal{L} = \{\mathcal{L}_{\rm Setup}(DB), \{\mathcal{L}_{\rm Query}(Q_i)~or~\mathcal{L}_{\rm Update}(Q_i)\}_{Q_i \in \bm{Q}}\}
\end{align*}
where $\mathcal{L}_{\rm Setup}$, $\mathcal{L}_{\rm Query}$, and $\mathcal{L}_{\rm Update}$ represent the profiles leaked when setting up the system, executing queries and updating the database, respectively.
Specifically, $\mathcal{L}_{\rm Update}$ could be $\mathcal{L}_{\rm Insert}$ or $\mathcal{L}_{\rm Delete}$.
%Note that the shuffling and re-randomisation operations are involved when executing queries and updating the database.
In the following, we analyse the specific information each CSP can learn from the received messages in each phase.

\paragraph{$\mathcal{L}_{\rm Setup}$}
When setting up the system, for the initial database $DB$, as shown in Algorithm \ref{alg:mcdb-setup}, the SSS gets the encrypted database $EDB$, and the IWS gets the group information $GDB$ and nonce information $NDB$.
In this phase, no data is sent to the RSS.
From $EDB$, the SSS learns the number of encrypted records $|EDB|$, the number of fields $F$, the length of each element $|e|$, and the length of tag $|tag|$.
From $NDB$ and $GDB$, the IWS learns $|NDB|$ ($|NDB|=|EDB|$), the length of each seed $|seed|$, the length of each nonce $|\bm{n}|$ ($|\bm{n}|=F|e|+|tag|$), the number of groups $|GDB|$, and the record identifiers $IL$ and $|(\bm{E}, \tau)^*|$ of each group.
In other words, the IWS learns the group information of each record in $EDB$.
Therefore, in this phase, the leakage $\mathcal{L}_{\rm Setup}(DB)$ learned by the SSS, IWS, and RSS can be respectively defined as:
%
\begin{align*}
    \mathcal{L}^{SSS}_{\rm Setup}(DB) = &\{|EDB|, \mathcal{L}_{rcd}\} \\
    \mathcal{L}^{IWS}_{\rm Setup}(DB) = &\{|NDB|, |\bm{n}|, |seed|, |GDB|,\\ & \{IL_{f, g}, |(\bm{E}_{f, g}, \tau)^*|\}_{(f, g) \in GDB}\} \\
    \mathcal{L}^{RSS}_{\rm Setup}(DB) = &\emptyset
\end{align*}
where $\mathcal{L}_{rcd}=\{F, |e|, |tag|\}$.


\paragraph{$\mathcal{L}_{\rm Query}$}
When processing queries, as mentioned in Algorithm \ref{alg:macdb-search} and \ref{alg:mcdb-shuffle}, the SSS gets the encrypted query $EQ$, $IL$ and encrypted nonces $EN$.
Based on them, the SSS can search over $EDB$ and gets the search result $SR$.
After shuffling, the SSS also gets the shuffled records $Ercds$ from the RSS.
From $\{EQ, IL, EN, SR, Ercds\}$, the SSS learns $\{Q.type, Q.f, |Q.e|, IL, |w|, |t|\}$, where $|t|=|seed|$.
%Specifically, $EDB(EQ)$ includes the number of matched records $|EDB(EQ)|$ and the location or identifier of each matched record.
In addition, the SSS can also infer the threshold $\tau$ ($\tau=|SR|$) and the number of distinct elements $|\bm{E}|$ ($|\bm{E}|=\frac{|IL|}{\tau}$) of the searched group.
%
The IWS only gets $(EQ.f, g, \eta)$ from the user, from which the IWS learns the searched field and group information of each query, and $|\eta|$ ($|\eta|=|Q.e|$).
%
The RSS gets the searched records $Ercds$, shuffled record identifies $IL'$, and new nonces $NN$ for shuffling and re-randomising.
From them, the RSS only learns $|Ercd|$ ($|Ercd|=|\bm{n}|$), $IL$ and $IL'$.
In summary,
%
\begin{align*}
	\mathcal{L}^{SSS}_{\rm Query}(Q) = &\{Q.f, Q.type, |Q.e|, Q.\bm{G}, |t|, |w|\} \\
    \mathcal{L}^{IWS}_{\rm Query}(Q) = &\{Q.f, g, |\eta|, |t|, |w|\} \\
    \mathcal{L}^{RSS}_{\rm Query}(Q) = &\{|Ercd|, IL, IL'\}
\end{align*}
where the group information $Q.\textbf{G}=\{g, IL, \tau, |\bm{E}|\}$.

\paragraph{$\mathcal{L}_{\rm Update}$}
Since different types of queries are processed in different manners, the SSS can learn if users are inserting, deleting or updating records, \ie $Q.type$.
As mentioned in Section \ref{subsec:update}, when inserting a real record, the user generates $W$ dummy ones, encrypts both the real and dummy records with $RcdEnc$, and sends them and their group information to the SSS and IWS, respectively.
Consequently, the SSS learns $W$, which represents the threshold or the number of elements of a group, and the IWS also learns the group information of each record.
Moreover, both the SSS and IWS can learn if the insert query introduces new elements that not belong to $U$ based on $|\bm{E}_{f, g}|$ or $|(\bm{E}_{f, g}, \tau_{f, g})^*|$.
The RSS only performs the shuffle operation.
Therefore, $\mathcal{L}_{\rm Insert}(Q)$ learned by each CSP is
\begin{align*}
	\mathcal{L}^{SSS}_{\rm Insert}(Q) = &\{W, \mathcal{L}_{rcd}\} \\
    \mathcal{L}^{IWS}_{\rm Insert}(Q) = &\{Grcd, \{|(\bm{E}_{f, g}, \tau_{f, g})^*|\}_{g_f \in Grcd}, W\} \\
    \mathcal{L}^{RSS}_{\rm Insert}(Q) = &\mathcal{L}^{RSS}_{\rm Query}(Q)
\end{align*}

Delete queries are performed as select queries in \framework, thus $\mathcal{L}_{\rm Delete} = \mathcal{L}_{\rm Query}$ for each CSP.

Above all,
\begin{align*}
	\mathcal{L}^{SSS} = &\{|EDB|, F, |e|, |tag|, |t|, |w|\\ &\{\{Q_i.f, Q_i.type, |Q_i.e|,  Q_i.\bm{G}\} ~or~ W\}_{Q_i \in \textbf{Q}}\} \\
    \mathcal{L}^{IWS} = &\{|NDB|, |GDB|, |\bm{n}|, |seed|, |w|, \\ &\{IL_{f, g}, |(\bm{E}_{f, g}, \tau)^*|\}_{(f, g) \in GDB}, \{\{Q_i.f, Q_i.g, |Q_i.e|\} \\ & ~or~ \{Grcd, \{|(\bm{E_{f, g}}, \tau_{f, g})^*|\}_{g_f \in Grcd}, W\}\}_{Q_i \in \textbf{Q}} \} \\
    \mathcal{L}^{RSS} = &\{|Ercd|, \{IL, IL'\}_{Q_i \in \bm{Q}}\}
\end{align*}

%Due to the groups, \framework additionally leaks the group information.
%We believe that it is much harder to infer the content of records and queries using the group information than using the search, access and size patterns. To prevent the adversary inferring more from the group information, on the one hand, the group function $GE$ should be defined independent of the plain data and the data distribution. On the other hand, as argued before, we should ensure each group contains a large number of distinct elements.

\subsection{Proof of Security}
Given the above leakage definition for each CSP, in this part, we prove adversaries do not learn anything beyond $\mathcal{L}^{csp}$ by compromising the CSP $csp$, where $csp$ could be the SSS, IWS, or RSS.
It is clear that adversaries cannot infer the search, access and size patterns, and forward and backward privacy of queries within a group from $\mathcal{L}^{csp}$.
Therefore, proving \framework only leaks $\mathcal{L}^{csp}$ to $csp$ indicates \framework protects the patterns and ensures forward and backward privacy within groups.

To prove \framework indeed only leaks $\mathcal{L}^{csp}$ to $csp$, we follow the typical method of using a real-world versus ideal-world paradigm \cite{Bost:2017:forward,CashJJJKRS14,KamaraPR12}.
The idea is that first we assume the CSP $csp$ is compromised by a Probabilistic Polynomial-Time (PPT) honest-but-curious adversary $\mathcal{A}$ who follows the protocol honestly as done by $csp$, but wants to learn more information by analysing the received messages and injecting malicious records.
Second, we build two experiments: $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ and $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A, S}, \mathcal{L}}(k)$, where $\Pi$ represents \framework.
In $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$, all the messages sent to $\mathcal{A}$ are generated as specified in \framework.
Whereas, in $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A, S}, \mathcal{L}}(k)$, all the messages are generated by a PPT simulator $\mathcal{S}$ that only has access to $\mathcal{L}^{csp}$.
That is, $\mathcal{S}$ ensures $\mathcal{A}$ only learns the information defined in $\mathcal{L}^{csp}$ from received messages in $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A, S}, \mathcal{L}}(k)$.
In the game, $\mathcal{A}$ chooses an initial database, triggers $Setup$, and adaptively issues \emph{select}, \emph{insert}, and \emph{delete} queries of its choice.
In response, either $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ or $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A, S}, \mathcal{L}}(k)$ is invoked to process the database and queries.
Based on the received messages, $\mathcal{A}$ distinguishes if they are generated by  $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ or $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A, S}, \mathcal{L}}(k)$.
If $\mathcal{A}$ cannot distinguish that with non-negligible advantage, it indicates $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ has the same leakage profile as $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A, S}, \mathcal{L}}(k)$.

%Otherwise, $\mathcal{A}_i$ can distinguish them based on the leakage out of $\mathcal{L}$.
%
\begin{mydef}
We say the dynamic SSE scheme is $\mathcal{L}$-adaptively-secure against the CSP $csp$, with respect to the leakage function $\mathcal{L}^{csp}$, if for any PPT adversary issuing a polynomial number of queries, there exists a PPT simulator $\mathcal{S}$, such that $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ and $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A, S}, \mathcal{L}}(k)$ are distinguishable with negligible probability $\textbf{negl}({k})$.
\end{mydef}

Herein, we acknowledge that \framework leaks the group information of queries and records and leaks whether the elements involved in select, insert and delete queries belong to $U$ or not.  For clarity, in the proof we assume there is only one group in each field, and omit the group processing. Moreover, we assume all the queries issued by $\mathcal{A}$ only involve elements in $U$.
In this case, the leakage learned by each CSP can be simplified into:
\begin{align*}
	\mathcal{L}^{SSS} = &\{|EDB|, F, |e|, |tag|, |t|, |w|\\ &\{\{Q_i.f, Q_i.type, |Q_i.e|\} ~or~ W\}_{Q_i \in \textbf{Q}}\} \\
    \mathcal{L}^{IWS} = &\{|NDB|, |\bm{n}|, |seed|, |w|, \{|(\bm{E}_{f}, \tau)^*|\}_{f \in [1, F]}, \\ &\{Q_i.f~or~W\}_{Q_i \in \textbf{Q}} \} \\
    \mathcal{L}^{RSS} = &\{|Ercd|, \{IL'\}_{Q_i \in \bm{Q}}\}
\end{align*}

%In the following, we assume $\mathcal{A}$ compromises the SSS and prove the security of \framework against the SSS.
%The security against the IWS and RSS can be proved in a similar way.

\begin{theorem}\label{the::SSS}
If $\Gamma$ is secure PRF, $\pi$ is a secure PRP, and $H'$ is a random oracle, \framework is a $\mathcal{L}$-adaptively-secure dynamic SSE scheme against the SSS.
\end{theorem}

\begin{proof}
To argue the security, as done in \cite{Bost:2017:forward,CashJJJKRS14,KamaraPR12}, we prove through a sequence of games.
The proof begins with $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$, which is exactly the real protocol, and constructs a sequence of games that differ slightly from the previous game and show they are indistinguishable.
Eventually we reach the last game $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A}, \mathcal{S}}(k)$, which is simulated by a simulator $\mathcal{S}$ based on the defined leakage profile $\mathcal{L}^{SSS}$.
By the transitive property of the indistinguishability, we conclude that $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ is indistinguishable from $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A}, \mathcal{S}}(k)$ and complete our proof.
Since $RcdDec$ is unrelated to CSPs, it is omitted in the games.
%
\begin{algorithm}[!htp]
\scriptsize
\caption{$\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k).RcdEnc(rcd, flag)$ $\|$ \fbox{$\mathcal{G}_1$}, \fbox{$\mathcal{G}_2$}, \fbox{$\mathcal{G}_3$}}
\label{proof::h1::enc}
\begin{algorithmic}[1]
\STATE $seed \stackrel{\$}{\lt} \{0,1\}^{|seed|}$
    \STATE $\bm{n} \lt \Gamma_{s_2} (seed)$ $\vartriangleleft$ \fbox{$\mathcal{G}_1$: $\bm{n} \lt \bm{Nonce}[seed]$}, where $\bm{n}= \ldots \parallel n_f \parallel \ldots \parallel n_{F+1}$, $|n_f|=|e|$ and $|n_{F+1}|=|tag|$
\FOR {each element $e_f \in rcd$}
    %\STATE $\sigma \lt Enc_{s_1}(e_f)$
    \STATE ${e^*_f} \lt Enc_{s_1}(e_f) \oplus n_f$  $\vartriangleleft$  {\fbox{$\mathcal{G}_3$: $e^*_f \lt \{0, 1\}^{|e|}$}}
\ENDFOR
\IF {$flag=1$}
    \STATE $S \stackrel{\$}{\leftarrow} \{0,1\}^{|e|}$
    \STATE $tag \leftarrow (H_{s_1}(S)||S )\oplus n_{F+1}$
    $\vartriangleleft$  {\fbox{$\mathcal{G}_3$: $tag \lt \{0, 1\}^{|tag|}$}}
\ELSE
    \STATE $tag \stackrel{\$}{\leftarrow} \{0,1\}^{|tag|}$
\ENDIF
\RETURN $Ercd=(e^*_1, \ldots, e^*_F, tag)$ and $(seed, \bm{n})$ %and $Grcd=(g_1$, ..., $g_F)$
\end{algorithmic}
\end{algorithm}
%
%
\begin{algorithm}[!htp]
\scriptsize
\caption{$\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k).Query(Q)$ $\|$ \fbox{$\mathcal{G}_1$}, \fbox{$\mathcal{G}_2$}, \fbox{$\mathcal{G}_3$}}
\label{h1:macdb-search}
\begin{algorithmic}[1]
	\STATE \underline{User: $QueryEnc(Q)$}
    %\STATE $g \leftarrow GE_{s_1}( Q.e )$  $\vartriangleleft$  {\fbox{$\mathcal{G}_2$: $g_f \lt \bm{Group}[Q.e]$}}
    \STATE $EQ.type \lt Q.type$, $EQ.f \lt Q.f$
    %\STATE $\sigma \lt Enc_{s_1}(Q.e)$
    \STATE $\eta \stackrel{\$}{\lt} \{0,1\}^{|e|}$
    \STATE $EQ.e^* \leftarrow Enc_{s_1}(Q.e) \oplus \eta$  $\vartriangleleft$  {\fbox{$\mathcal{G}_3$: $EQ.e^* \lt \{0, 1\}^{|e|}$}}
    \STATE Send $EQ=(type, f, op, e^*)$ to the SSS
    \STATE Send $(EQ.f, \eta)$ to the IWS

~\\


\STATE \underline{IWS: $NonceBlind(EQ.f, \eta)$}
    \STATE $EN \leftarrow \emptyset$
    %\STATE $IL \leftarrow GDB(EQ.f, g)$
    \STATE \fbox{$\mathcal{G}_2$: Randomly put $\tau_f$ record identifiers into $\bm{I}$}
    \FOR {each $id \in NDB$ }
        \STATE $(seed, \bm{n}) \leftarrow NDB(id)$, where $\bm{n}= \ldots ||n_{EQ.f}|| \ldots $ and $|n_{EQ.f}|=|\eta|$    $\vartriangleleft$   \fbox{Deleted in $\mathcal{G}_2$}
        \STATE  ${w} \lt H'(n_{EQ.f} \oplus \eta)$   $\vartriangleleft$    \fbox{$\mathcal{G}_2$:~~\begin{minipage}[c][1.0cm][t]{4.5cm}{\textbf{if} $id \in \bm{I}$ \\ $w_{id} \lt H'(EDB(id, EQ.f) \oplus EQ.e^*)$ \\ \textbf{else} \\ $w_{id} \lt \{0, 1\}^{|w|}$ } \end{minipage}}
        \STATE  $t \lt \eta \oplus seed$   $\vartriangleleft$  {\fbox{$\mathcal{G}_3$: $t \lt \{0, 1\}^{|seed|}$}}
        \STATE  $EN(id) \leftarrow (w, t)$
    \ENDFOR
    \STATE Send the encrypted nonce set $EN=((w, t), \ldots)$ to the SSS

~\\
%
\STATE \underline{SSS: $Search(EQ, EN)$}
    \STATE $SR \leftarrow \emptyset$
    \FOR {each $id \in EDB$}
        \IF {$H'(EDB(id, EQ.f) \oplus EQ.e^*) = EN(id).w$}
             \STATE $SR \leftarrow SR \cup (EDB(id), EN(id).t)$
        \ENDIF
    \ENDFOR
    \STATE Send the search result $SR$ to the user
		
	\end{algorithmic}
\end{algorithm}
%
%
\begin{algorithm}[!ht]
\scriptsize
\caption{$\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k).Shuffle()$ $\|$ \fbox{$\mathcal{G}_1$}, \fbox{$\mathcal{G}_2$}, \fbox{$\mathcal{G}_3$}}
\label{h1:mcdb-shuffle}
\begin{algorithmic}[1]
\STATE \underline{IWS: $PreShuffle()$}
	\STATE {$IL' \leftarrow \pi(NDB)$}
	%\STATE Shuffle the seeds indexed by $IL$ based on $IL'$
	%\STATE Update the indexes of affected groups in $GDB$
	\FOR {each $id \in IL'$}
		\STATE $seed \stackrel{\$}{\leftarrow} \{0, 1\}^{|seed|}$
        \STATE $\bm{n}' \lt \Gamma_{s_2}(seed)$  $\vartriangleleft$ \fbox{$\mathcal{G}_1$: $\bm{n}' \lt \bm{Nonce}[seed]$} %\tikzmark{end2}
		\STATE $NN(id) \leftarrow NDB(id).\bm{n} \oplus \bm{n}' $   $\vartriangleleft$ \fbox{$\mathcal{G}_3$: $NN(id) \lt \{0, 1\}^{|\bm{n}|}$}
		\STATE $NDB(id)\leftarrow (seed, \bm{n}')$
	\ENDFOR
	\STATE Send $(IL', NN)$ to the RSS.

~\\~
\STATE{\underline{RSS: $Shuffle(Ercds, IL', NN)$}}
	\STATE Shuffle $Ercds$ based on $IL'$
	\FOR {each $id \in IL'$}
	\STATE {$Ercds(id) \leftarrow Ercds(id) \oplus NN(id)$}   $\vartriangleleft$ \fbox{$\mathcal{G}_3$: $Ercds(id) \lt \{0, 1\}^{|\bm{n}|}$}
	\ENDFOR
	\STATE Send $Ercds$ to the SSS.
\end{algorithmic}
\end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\smallskip
\noindent\textbf{Game $\mathcal{G}_1$}: Comparing with $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$, the difference in $\mathcal{G}_1$ is that the PRF $\Gamma$ for generating nonces, in $RcdEnc$ and $PreShuffle$ algorithms, is replaced with a mapping \textbf{Nonce}.
Specifically, as shown in Algorithm \ref{proof::h1::enc} and \ref{h1:mcdb-shuffle}, for each unused $seed$ (the length of seed is big enough), a random string of length $F|e|+|tag|$ is generated as the nonce, stored in \textbf{Nonce}, and then reused thereafter.
This means that all of the $\bm{n}$ are uniform and independent strings.
In this case, the adversarial distinguishing advantage between $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ and $\mathcal{G}_1$ is exactly the distinguishing advantage between a truly random function and PRF.
%Indeed, the distinguishing advantage between a truly random function and PRF is negligible.
Thus, this change made negligible difference between between $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ and $\mathcal{G}_1$, \ie
\[
\centerline { $|{\rm Pr}[\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)=1] - {\rm Pr}[\mathcal{G}_1=1]| \leq \textbf{negl}({k})$}
\]
where ${\rm Pr}[\mathcal{G}=1]$ represents the probability of that the messages received by $\mathcal{A}$ are generated by $\mathcal{G}$.

\noindent\textbf{Game $\mathcal{G}_2$}:
From $\mathcal{G}_1$ to $\mathcal{G}_2$, $w$ is replaced with a random string, rather than generated via $H'$.
However, it is necessary to ensure $\mathcal{A}$ gets $\tau_f$ matched records after searching over $EDB$, since that is the leakage $\mathcal{A}$ learns, where $\tau_f$ is the threshold of the searched field.
To achieve that, the experiment randomly picks $\tau_f$ witnesses and programs their values.
Specifically, as shown in Algorithm \ref{h1:macdb-search}, the experiment first randomly picks a set of record identifiers $\bm{I}$, where $|\bm{I}|=\tau_f$.
Second, for each identifier $id \in \bm{I}$, the experiment programs $w_{id} \lt H'(EDB(id, EQ.f) \oplus EQ.e^*)$.
By doing so, the records identified by $\bm{I}$ will match the query.
For the identifier $id \notin \bm{I}$, $w_{id} \lt \{0, 1\}^{|w|}$.

The only difference between $\mathcal{G}_2$ and $\mathcal{G}_1$ is the generation of $w$.
In the following, we see if $\mathcal{A}$ can distinguish the two games based on $w$.
In $\mathcal{G}_2$,
%
\begin{align}\notag
  For~id \in \bm{I}, ~w_{id} &\lt H'(EDB(id, EQ.f) \oplus EQ.e^*)  \\ \notag
  For~id \notin \bm{I}, ~w_{id} &\lt \{0, 1\}^{|w|}
\end{align}
%
Recall that in $\mathcal{G}_1$.
\begin{equation}\notag
  w_{id} \lt H'(n_{EQ.f} \oplus \eta)
\end{equation}
%
In $\mathcal{G}_1$, $n_{EQ.f}$ and $\eta$ are random strings.
In $\mathcal{G}_2$, due to the one-time pad encryption in $RcdEnc$ and $QueryEnc$, $EDB(id, EQ.f)$ and $EQ.e^*$ are indistinguishable from random strings.
Thus, we can say for $id \in \bm{I}$ $w_{id}$ is generated in the same way as done in $\mathcal{G}_1$. 
For $id \notin \bm{I}$, $w_{id}$ is a random string in $\mathcal{G}_2$, whereas in $\mathcal{G}_1$  $w_{id}$ is generated by deterministic $H'$. 
It seems $\mathcal{A}$ could easily distinguish $\mathcal{G}_2$ and $\mathcal{G}_1$, since $\mathcal{G}_1$ outputs the same $w$ for the same input, whereas $\mathcal{G}_2$ does not.
Indeed, in $\mathcal{G}_1$ the inputs to $H'$, $n_{EQ.f}$ and $\eta$, are random strings, thus the probability of getting the same input for $H'$ is negligible, making $H'$ indistinguishable from a uniform sampling. 
Thus, in both cases $w_{id}$ in $\mathcal{G}_2$ is indistinguishable from $w_{id}$ in $\mathcal{G}_1$. 

Next, we discuss if $\mathcal{A}$ can distinguish the two games based on $SR$.
The leakage of $SR$ includes the identifier of each matched records and $|SR|$.
Due to the padding, $|SR|=|\bm{I}|=\tau_f$, which means the two games are indistinguishable based on $|SR|$.
In $\mathcal{G}_1$, the identifiers of matched records are determined by the shuffle operations performed for the previous query.
In $\mathcal{G}_2$, the identifiers of matched records are randomly picked.
Thus, the distinguishing advantage between $\mathcal{G}_1$ and $\mathcal{G}_2$ based on the identifiers is exactly the distinguishing advantage between a truly random permutation and PRP, which is negligible.

Above all, we have
\[
\centerline { $|{\rm Pr}[\mathcal{G}_2=1] - {\rm Pr}[\mathcal{G}_1=1]| \leq \textbf{negl}(k)$}
\]

\noindent\textbf{Game $\mathcal{G}_3$}:
The difference between $\mathcal{G}_2$ and $\mathcal{G}_3$ is that all the XORing operations, such as the generation of $e^*$, $Q.e^*$, and $t$, are replaced with randomly sampled strings (The details are shown in Algorithms \ref{proof::h1::enc}, \ref{h1:macdb-search}, and \ref{h1:mcdb-shuffle}).
Since sampling a fixed-length random string is indistinguishable from the one-time pad encryption,
we have
\[
\centerline { ${\rm Pr}[\mathcal{G}_3=1] = {\rm Pr}[\mathcal{G}_2=1] $}
\]

%
%%Simulation%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[!htp]
\scriptsize
\caption{$\mathcal{S}.RcdEnc(\mathcal{L}_{rcd}$)}
\label{proof::ideal::enc}
\begin{algorithmic}[1]
	\STATE \tgrey{$seed \stackrel{\$}{\lt} \{0,1\}^{|seed|}$}
	\STATE \tgrey{$\bm{n} \lt \bm{Nonce}[seed]$}
    \FOR {each $f \in [1, F]$}
        %\STATE {$g_f \lt \bm{Group}[e_f]$} %\tikzmark{startSenc}\tikzmark{endSenc}
        \STATE ${e^*_f} \lt \{0, 1\}^{|e|}$
    \ENDFOR
	\STATE 	{$tag \stackrel{\$}{\leftarrow} \{0,1\}^{|tag|}$}
	\RETURN {$Ercd=(e^*_1, \ldots, e^*_F, tag)$} and \tgrey{$(seed, \bm{n})$} %and $Grcd=(g_1$, \ldots, $g_F)$
\end{algorithmic}
\end{algorithm}
%\Textbox[5.5cm]{startSenc}{endSenc}{grouping information from ideal leakage}

%
\begin{algorithm}[!htp]
\scriptsize
\caption{$\mathcal{S}.Query(\mathcal{L}^{SSS}_{Query})$}
\label{ideal:macdb-search}
\begin{algorithmic}[1]
	\STATE \underline{User: $QueryEnc(\mathcal{L}^{SSS}_{Query})$}
    %\STATE $g \lt \bm{Group}[Q.e]$
    \STATE $EQ.type \lt Q.type$, $EQ.f \lt Q.f$
    \STATE \tgrey{$\eta \stackrel{\$}{\lt} \{0,1\}^{| e |}$}
    \STATE $EQ.e^* \leftarrow \{0, 1\}^{|e|}$
    \STATE Send $EQ=(type, f, op, e^*)$ to the SSS
    \STATE \tgrey{Send $(EQ.f, \eta)$ to the IWS}

~\\

\STATE \underline{IWS: $NonceBlind(\mathcal{L}^{SSS}_{Query})$}
    \STATE $EN \leftarrow \emptyset$
    %\STATE $IL \leftarrow GDB(EQ.f, g)$
    \STATE Randomly put $\tau_f$ records identifers into $\bm{I}$
    \FOR {each $id \in [1, |EDB|]$ }
        \IF{$id \in \bm{I}$}
            \STATE  ${w} \lt H'(EDB(id, EQ.f) \oplus EQ.e^*)$
        \ELSE
            \STATE  ${w} \lt \{0, 1\}^{|w|}$
        \ENDIF
        \STATE  $t \lt \{0, 1\}^{|seed|}$
        \STATE  $EN(id) \leftarrow (w, t)$
    \ENDFOR
    \STATE Send the encrypted nonce set $EN=((w, t), \ldots)$ to the SSS

~\\
%
\STATE \underline{SSS: $Search(EQ, EN)$}
    \STATE $SR \leftarrow \emptyset$
    \FOR {each $id \in EDB$}
        %\STATE $\nu \lt $
        \IF {$H'(EDB(id, EQ.f) \oplus EQ.e^*) = EN(id).w$ }
             \STATE $SR \leftarrow SR \cup (EDB(id), EN(id).t)$
        \ENDIF
    \ENDFOR
    \STATE Send the search result $SR$ to the user
		
	\end{algorithmic}
\end{algorithm}
%

\begin{algorithm}
\scriptsize
\caption{$\mathcal{S}.Shuffle(\mathcal{L}^{SSS}_{Query})$}
\label{proof::ideal::shuffle}
\begin{algorithmic}[1]
\STATE \underline{IWS: $PreShuffle()$}
    \STATE \tgrey{$IL' \leftarrow RP (NDB)$}
    \FOR {\tgrey{each $id \in IL'$}}
        \STATE \tgrey{$seed \stackrel{\$}{\leftarrow} \{0, 1\}^{|seed|}$}
        \STATE \tgrey{$\bm{n'} \leftarrow  \bm{Nonce}[seed]$}
        \STATE \tgrey{$NN(id) \leftarrow \{0, 1\}^{|\bm{n}|}$}
        \STATE \tgrey{$NDB(id)\leftarrow (seed, \bm{n'})$}
    \ENDFOR
    \STATE \tgrey{Send $(IL', NN)$ to the RSS.}

~\\

\STATE{\underline{RSS: $Shuffle(\mathcal{L}^{SSS}_{Query})$}}
    \STATE \tgrey{Shuffle $Ercds$ based on $IL'$}
    \FOR {each $id \in IL$}
        \STATE $Ercds(id) \leftarrow \{0, 1\}^{|\bm{n}|} $
    \ENDFOR
    \STATE Send $Ercds$ to the SSS.
\end{algorithmic}
\end{algorithm}
%

%\smallskip
\noindent\textbf{$\textbf{Ideal}^{\rm \Pi}_{\mathcal{A}, \mathcal{S}, \mathcal{L}}(k)$}:
From $\mathcal{G}_3$ to the final game, we just replace the inputs to $RcdEnc$, $Query$ and $Shufle$ algorithms with $\mathcal{L}^{SSS}$.
Moreover, for clarity, we fade the operations unrelated to the SSS.
From Algorithms \ref{proof::ideal::enc}, \ref{ideal:macdb-search}, and \ref{proof::ideal::shuffle}, it is easy to observe that the messages sent to $\mathcal{A}$, \ie $\{Ercd, EQ, EN, Ercds\}$, can be easily simulated by only relying on $\mathcal{L}^{SSS}$.
Here we have:

\[
{\rm Pr}[\textbf{Ideal}^{\rm \Pi}_{\mathcal{A},\mathcal{S}, \mathcal{L}}(k)=1]={\rm Pr}[\mathcal{G}_3=1]
\]

By combining all the distinguishable advantages above, we get:
\[
|{\rm Pr}[\textbf{Ideal}^{\rm \Pi}_{\mathcal{A},\mathcal{S}, \mathcal{L}}(k)=1]- {\rm Pr}[\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)=1]| < \textbf{negl}(k)
\]

%\ref{alg:proof-mcdb-setup},
In $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A},\mathcal{S}, \mathcal{L}}(k)$, $\mathcal{A}$ only learns $\mathcal{L}_{rcd}$ and $\mathcal{L}^{SSS}_{Query}$.
The negligible advantage of a distinguisher between $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ and $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A},\mathcal{S}, \mathcal{L}}(k)$ indicates that \framework also only leaks $\mathcal{L}_{rcd}$ and $\mathcal{L}^{SSS}_{Query}$.

Although the above simulation does not include the $Setup$ and updating phases, it is clear that the two phases mainly rely on $RcdEnc$ algorithm, which has been proved only leaks $\mathcal{L}_{rcd}$ to the SSS.
From $Setup$ phase, $\mathcal{A}$ only gets $EDB$, and each record in $EDB$ is encrypted with $RcdEnc$.
Thus, $\mathcal{A}$ only learns $|EDB|$ and $\mathcal{L}_{rcd}$ in this phase.
Similarly, $\mathcal{A}$ only gets $W+1$ encrypted records in $Insert$ algorithm.
Therefore, in addition to $\mathcal{L}_{rcd}$, it only learns $W$, which is equal to $|\bm{E}|$ or $\tau$ of a group.
For delete queries, $\mathcal{A}$ learns $\mathcal{L}^{SSS}_{Query}$ since they are first performed as select queries.
As proved above, the tags are indistinguishable from random strings, meaning the returned tags do not leak additional information.
\end{proof}

\begin{theorem}\label{the::IWS}
If $ENC$ is semantically secure, \framework is a $\mathcal{L}$-adaptively-secure dynamic SSE scheme against the IWS.
\end{theorem}

\begin{proof}
Herein, we also assume all the records are in one group.
In this case, the IWS gets $(seed, \bm{n})$ for each record and $(\bm{E}_f, \tau_f)^*$ for each field when setting up the database, gets $(Q.f, \eta)$ when executing queries, and gets updated $(\bm{E}_f, \tau_f)^*$ when inserting records.
Note that the IWS can generate $\bm{n}$ by itself since it has the key $s_2$.
Considering $seed$ and $\eta$ are random strings, from $\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)$ to $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A}, \mathcal{S}, \mathcal{L}}(k)$ we just need one step.
Specifically, given $\mathcal{L}^{IWS}$, in $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A}, \mathcal{S}, \mathcal{L}}(k)$, $\mathcal{S}$ just needs to simulate $(\bm{E}_f, \tau_f)^*$ with $|(\bm{E}_f, \tau_f)^*|$-bit random strings in $Setup$ and $Insert$ algorithms.
Given $ENC$ is semantically secure, we have
\[
|{\rm Pr}[\textbf{Ideal}^{\rm \Pi}_{\mathcal{A},\mathcal{S}, \mathcal{L}}(k)=1]- {\rm Pr}[\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)=1]| < \textbf{negl}(k)
\]
\end{proof}

\begin{theorem}\label{the::RSS}
\framework is a $\mathcal{L}$-adaptively-secure dynamic SSE scheme against the RSS.
\end{theorem}

\begin{proof}
In \framework, the RSS is only responsible for shuffling and re-randomising records after each query.
For the shuffling and re-randomising, it gets encrypted records, $IL'$ and $NN$.
Here we also just need one step to reach $\textbf{Ideal}^{\rm \Pi}_{\mathcal{A}, \mathcal{S}, \mathcal{L}}(k)$.
Given $\mathcal{L}^{RSS}$, as done in the above \textbf{Game $\mathcal{G}_3$}, $\mathcal{S}$ needs to replace $e^*$ and $tag$ in $RcdEnc$ with $|e|$-bit and $|tag|$-bit random strings respectively and simulate each element in $NN$ with a $|Ercd|$-bit random string in $PreShuffle$.
As mentioned, since sampling a fixed-length random string is indistinguishable from the one-time pad encryption, we have
\[
|{\rm Pr}[\textbf{Ideal}^{\rm \Pi}_{\mathcal{A},\mathcal{S}, \mathcal{L}}(k)=1] = {\rm Pr}[\textbf{Real}^{\rm \Pi}_{\mathcal{A}}(k)=1]|
\]
\end{proof}


==> PMcDb_arXiv/setup/macros.tex <==
%------------------------Custom Commands----------------------%
% = = = Latin Short-forms (ie, eg, etc, et al)
\usepackage{xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\supra}{\textit{Supra}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}
% \mathchardef\-="2D
\mathchardef\mhyphen="2D


% = = = Arrow -> (\lt)
\newcommand{\rt}{\rightarrow}
\newcommand{\lt}{\leftarrow}
\newcommand{\rnd}{\stackrel{\$}{\leftarrow}}

\newcommand{\framework}{\textsl{\mbox{P-McDb}}\xspace}
\newcommand{\kw}[1]{\textsf{#1}}

% = = = Colored text (textblue)
%\newcommand{\textblue}[1]{{#1}}
\newcommand{\tblue}[1]{\textcolor{blue}{#1}}
\newcommand{\tred}[1]{\textcolor{red}{#1}}
\newcommand{\tgrey}[1]{\textcolor{lightgray}{#1}}

\newcommand{\xiangfu}[1]{{\color{blue} #1}}
\newcommand{\attention}[1]{{\color{red} #1}}


% = = = Compact Lists (compactlist, compactlistn)
\newenvironment{compactlist}
  {\begin{itemize}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}}
  {\end{itemize}}

\newenvironment{compactlistn}
  {\begin{enumerate}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}}
  {\end{enumerate}}

\renewcommand{\labelitemi}{$\bullet$}

\newcommand{\pparagraph}[1]{\medskip \noindent \textbf{#1\ }}
\renewcommand{\paragraph}[1]{\medskip \noindent \textbf{#1.\ }}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


\newtheorem{mydef}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}

\iffalse
\newcommand\tikzmark[1]{%
  \tikz[remember picture,overlay]\node[inner xsep=4pt] (#1) {};}
\newcommandtwoopt\Textbox[5][3cm][4.5cm]{%
\begin{tikzpicture}[remember picture,overlay]
  \coordinate (aux) at ([xshift=#1]#4);
  \node[inner ysep=3.3pt,yshift=0.5ex,draw=black,thick,
    fit=(#3) (aux),baseline]
    (box) {};
  \node[text width=#2,anchor=south east,
    font=\sffamily\scriptsize,align=right]
    at (box.south east) {#5};
\end{tikzpicture}%
}
\fi


==> PMcDb_arXiv/setup/packages.tex <==
\usepackage{amsmath}
\usepackage{amssymb}         % used for checkmark and times
\usepackage{amsthm}
\usepackage{graphicx}        % standard LaTeX graphics tool
                             % when including figure files
\usepackage{footnote}
%\usepackage[bottom]{footmisc}% places footnotes at page bottom
\usepackage[hang,flushmargin]{footmisc}
\usepackage{marvosym}
\usepackage{epstopdf}
\usepackage{epsfig}
\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage[noend]{algorithmic}
%\usepackage{subcaption}
%\usepackage{wasysym}         % used for checkmark and times
%\usepackage{dingbat}
\usepackage{diagbox}
\usepackage{subfigure}
%\usepackage[hyphens]{url}
\usepackage{hyperref}
%\usepackage{breakurl}
%\usepackage{dsfont}
\usepackage{todonotes}
\usepackage{color}
%\usepackage{makecell}
%\usepackage{tablefootnote}
\usepackage{bm} % formula bold
%\usepackage{listings}
\usepackage{multirow}

\usepackage{twoopt}
\usepackage{tikz}
\usetikzlibrary{fit}

\ifCLASSOPTIONcompsoc
  % IEEE Computer Society needs nocompress option
  % requires cite.sty v4.0 or later (November 2003)
  \usepackage[nocompress]{cite}
\else
  % normal IEEE
  \usepackage{cite}
\fi


==> sections/table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{The computation and communication overhead in \framework. }
\label{tbl:complexity}
\begin{tabular}{|l|l|l|l|}
\hline
\emph{Method }          & \textbf{Operation}       & \textbf{Computation}                                                                                                                                                                         & \textbf{Communication}           \\ \hline
\multirow{3}{*}{P-McDb} & Search                   & \begin{tabular}[c]{@{}l@{}}User: $XOR_{\lambda}+Enc_{\lambda}$\\ WSS: $PRG_{m\lambda}+XOR_{\lambda}+Hash_{\lambda}+XOR_{|seed|}$\\ SSS: $XOR_{\lambda}+hash_{\lambda}$\end{tabular} & $\lambda + |seed|$ bits \\ \cline{2-4}
                        & Decryption               & User: $XOR_{|seed|}+PRG_{m\lambda}+m(XOR_{\lambda}+Enc^{-1}_{\lambda})$                                                                                                             & $m\lambda + |seed|$     \\ \cline{2-4}
                        & Shuffle                  & \begin{tabular}[c]{@{}l@{}}WSS: $PRG_{m\lambda} + mXOR_{\lambda}$\\ SSS: $2mXOR_{\lambda}$\end{tabular}                                                                             & $2m\lambda$ bits        \\ \hline
\multirow{3}{*}{PPQED}  & Search                   & \begin{tabular}[c]{@{}l@{}}User: $Sub_N$\\ C1: $HA+ \lambda HE_k+SC$\\ C2: $HE + HD_k$\end{tabular}                                                                                  & $2k+?$                  \\ \cline{2-4}
                        & Decryption               & User: $m(HD_k+Sub_N)$                                                                                                                                                               & $2mk$                   \\ \cline{2-4}
                        & Oblivious data retrieval & \begin{tabular}[c]{@{}l@{}}C1: $m(HA+HE_k)$\\ C2: $mHD_k$\end{tabular}                                                                                                              & $3mk$                   \\ \hline
\end{tabular}

$XOR_{\lambda}$, $Enc_{\lambda}$, $Hash_{\lambda}$ and $Enc^{-1}_{\lambda}$ represent the computation overhead to perform these operations over $\lambda$ bits data, respectively. $PRG_{m\lambda}$ represents the computation overhead to generate a $m\lambda$-bit nonce.
\end{table*}
